Think about it! Improving defeasible reasoning by first modeling the question scenario

Defeasible reasoning is the mode of reasoning where conclusions can be overturned by taking into account new evidence. Existing cognitive science literature on defeasible reasoning suggests that a person forms a mental model of the problem scenario before answering questions. Our research goal asks whether neural models can similarly benefit from envisioning the question scenario before answering a defeasible query. Our approach is, given a question, to have a model first create a graph of relevant influences, and then leverage that graph as an additional input when answering the question. Our system, CURIOUS, achieves a new state-of-the-art on three different defeasible reasoning datasets. This result is significant as it illustrates that performance can be improved by guiding a system to "think about" a question and explicitly model the scenario, rather than answering reflexively. Code, data, and pre-trained models are located at https://github.com/madaan/thinkaboutit.

==> mercurie/sections-old/abstract.tex <==
\begin{abstract}
Question-answering (QA) often involves reasoning about {\it chains of influence}.
For example, to answer "Can storms increase beach erosion?" a person might reason
that storms produce bigger waves, resulting in more erosion (hence "yes").
From a cognitive science perspective, a person appears to form a ``mental model''
of the scenario behind the question before answering it.
Our research goal asks whether neural models can similarly benefit
from envisioning the QA scenario before answering a question.
Our approach is, given a question, to have a model first create a graph
of relevant influences,
and then effectively leverage that graph as an additional input when answering the question.
We find that \ours achieves a new state-of-the-art on three different defeasible reasoning datasets, as well as now producing justifications for its answers.
This result is significant as it suggests model performance in other contexts may similarly be improved by guiding them to ``think about'' a question and explicitly model the scenario, rather than answering reflexively.
\end{abstract}


==> mercurie/sections-old/better_graphs.tex <==
\section{Improving the graphs for defeasible inference}
\label{sec:graphgen}
We evaluate the graphs produced by \calM for defeasible reasoning using human evaluators. Two human judges evaluated 100 graphs produced by \calM. 
The judges found that all the graphs had the correct structure, but 70\% of them had \textit{repeated} nodes with the same information.

Each node in an influence graph plays a specific role (e.g., positive contextualizer or mediator). Thus, repeated nodes violate the semantic structure of a graph.
Additionally, they also reduce the amount of information carried by each graph.
For defeasible reasoning, we focus on reducing this repetition of nodes in each graph.
We note that we do not utilize the edge structure of the graph for this work or take feedback on it.
The structure of the graphs is assumed to be fixed.
Our intuition is that reducing the number of repeated nodes will improve the quality of these graphs, making them more useful for downstream tasks.
To be consistent across tasks, we refer to such graphs with repeated nodes as being \textit{incorrect graphs}.


\SetKwInput{KwGiven}{Given}
\SetKwInput{KwInit}{Init}
\begin{algorithm}[!h]
\SetAlgoLined
\KwGiven{Inference graphs G generated by \GEN, and G* generated by \GEN*}
\KwResult{Training data for \CORR}
\KwInit{$\mathcal{D} \gets [ ]$}
\For{$i \gets 1, 2, \ldots, |\mathcal{M}|$}{
$F_{G_i} = feedback(G_i)$ \;
$F_{G_i}* = feedback(G_i*)$\;
\uIf{$F_{G_i} \not = \emptyset$ and $F_{G_i}* = \emptyset$}{
\tcc{$G_i$ has problems, $G_i*$ is good}
$\mathcal{D} = \mathcal{D} \cup (G_i, F_{G_i}, G_i*)$\;
} \uElseIf {$F_G = \emptyset$ and $F_G* = \emptyset$} {
\tcc{Both $G_i$ and $G_i*$ are good}
$\mathcal{D} = \mathcal{D} \cup (G_i, \text{No issues, looks good}, G_i*)$\;
}
}
\KwRet{$\mathcal{D}$}
\caption{Generating training data for \CORR using human feedback.}
\label{alg:alg-train-for-corr}
\end{algorithm}

\subsection{Automating human-like feedback}
\label{sec:automate-human-like-feedback}
We observed that humans found it cognitively challenging to look at multiple nodes and check for the consistency of nodes and repetition of content across multiple unrelated or opposite polarity nodes. In contrast, prior work on assembling structure edit commands relies on the relative simplicity of the structure (such as in an SQL query), allowing targeted feedback. This is not possible in our case, owing to the sizeable cognitive load of manually labeling each node while maintaining structural consistency. Therefore, using human annotations, we devised a simple rule-based system $F$ that uses token-based overlap to detect repetitions while preventing spurious matches due to negation. 
Figures \ref{fig:snliexample}, \ref{fig:atomicexample}, and \ref{fig:socialexample} show examples of various kinds of inconsistencies and the corresponding feedback.


\subsubsection{Automating expected corrected graph}
\label{sec:automate-expected-corrected-graph}
Ideally, it would be desirable to have training data that provides a \textit{fixed graph} corresponding to each incorrect graph. 
However, we realized that manually fixing incorrect graphs is not scalable, as it requires identifying repeated nodes and then coming up with a label that would remove the repetitions across the graph.
We circumvent this issue by training another version of graph generator \GENS.
The training process of \GENS closely follows that of \GEN: we set the input to $P \Vert H \Vert S \Vert T$ and the output to $G$.
Note that the only difference here from \GEN is that the generation is now additionally conditioned on the edges, leading to more diverse and possibly less noisy graphs.

During inference, we obtain a graph for the defeasible query \phu by setting passage = \pre, hypothesis = \hypo, and situation = \upd, as discussed. Figure~\ref{fig:deftrain} shows the details of the training process.

We further note that such conditioning is not possible for the general case since the graph edges are not available with defeasible queries.

We use T5-11B~\cite{raffel2020exploring} as our graph generator \GEN, feedback graph generator \GENS, as well as graph corrector \CORR.
% \begin{figure*}
% \centering
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[width=.80\linewidth]{imgs/snli_bad.pdf}
%   \caption{\textit{C-, C+ and S,S- are overlapping.}}
% \end{minipage}%
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[width=.8\linewidth]{imgs/social_bad.pdf}
%   \caption{\textit{C-,C+,S,S-  and M-, M+, H+ are overlapping.}}
% \end{minipage}
%   \captionof{figure}{Incorrect graphs generated by \GEN for SNLI (left) SOCIAL domains of Defeasible. The feedback on each graph is mentioned in caption, and we provide the fixed versions of these graphs in the Appendix.}
%   \label{fig:feedbackexample}
% \end{figure*}


==> mercurie/sections-old/custom_commands.tex <==
\definecolor{Red}{rgb}{1,0,0}
\definecolor{Green}{rgb}{0.4,1,0.2}
\definecolor{Blue}{rgb}{0,0,1}
\definecolor{Red}{rgb}{0.9,0,0}
\definecolor{Orange}{rgb}{1,0.5,0}
\definecolor{yellow}{rgb}{0.65,0.6,0}
\definecolor{cadmiumgreen}{rgb}{0.2, 0.7, 0.24}
\newcommand{\V}[1]{\mathbf{#1}}
\newcommand{\C}[1]{\mathcal{#1}}
\newcommand{\red}[1]{\textcolor{Red}{#1}}
\newcommand{\green}[1]{\textcolor{cadmiumgreen}{#1}}
\newcommand{\nk}[1]{\textcolor{Red}{[#1 \textsc{--Niket}]}}
\newcommand{\corr}[2]{\textbf{\textcolor{red}{\sout{#1} #2}}}
\newcommand{\am}[1]{\textcolor{Orange}{[#1 \textsc{--Aman}]}}
\newcommand{\dheeraj}[1]{\textcolor{Blue}{[#1 \textsc{--Dheeraj}]}}
\newcommand{\sm}[1]{\textcolor{Orange}{[#1 \textsc{--SM}]}}
%\newcommand{\yyc}[1]{\textcolor{Blue}{[#1 \textsc{--YY}]}}
%\newcommand{\yyc}[2]{\textcolor{blue}{\sout{#1} #2}}
%\newcommand{\yy}[1]{\textcolor{cyan}{[#1 \textsc{--YY}]}}
\newcommand{\notes}[1]{\textcolor{Red}{[#1 \textsc{--notes}]}}
\newcommand{\ed}[1]{\textcolor{cyan}{[#1 \textsc{--Ed}]}}
\newcommand{\lasha}[1]{\textcolor{yellow}{[#1 \textsc{--Abhilasha}]}}
\newcommand{\ar}[1]{\textcolor{red}{\bf\small [#1 --Abhilasha]}}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand\given[1][]{\:#1\vert\:}

% \newcommand{\C}[1]{$\mathcal{#1}$\xspace}

\newcommand{\X}[1]{\mathbf{\mathrm{S}}}
\newcommand{\Z}[1]{\mathbf{\mathrm{C^-}}}
\newcommand{\VV}[1]{\mathbf{\mathrm{C^+}}}
\newcommand{\W}[1]{\mathbf{\mathrm{M^-}}}
\newcommand{\U}[1]{\mathbf{\mathrm{S^-}}}
\newcommand{\Y}[1]{\mathbf{\mathrm{M^+}}}
\newcommand{\LL}[1]{\mathbf{\mathrm{H^-}}}
\newcommand{\M}[1]{\mathbf{\mathrm{H^+}}}
\newcommand{\proscript}[1]{ProScript}


% "Z": [  "C-
%         "V": [ "C+
%         "X": [ "S :
%         "W": [ "M-
%         "U": [ "S- :
%         "Y": [ "M+ :
%         "A": [ "O+ :
%         "D": [ "O+ :
%Constants
\newcommand{\numgraphs}{2107\xspace}
\newcommand{\numpassages}{379\xspace}
\newcommand{\numquestions}{40.7K\xspace}
\newcommand{\grn}[1]{\textcolor{cadmiumgreen}{#1}}


%Hyperparams
\newcommand{\lrate}{\textcolor{Red}{LR-HERE} }
\newcommand{\dropout}{\textcolor{Red}{DROPOUT-HERE} }
% \newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\rdim}[1]{\in \mathbb{R}^{#1}}
\newcommand{\cadmiumgreen}[1]{\textcolor{cadmiumgreen}{#1}}

%\newcommand{\helps}{\stackrel{(+)}\longrightarrow}
% \newcommand{\hurts}{\stackrel{(-)}\longrightarrow}
% \newcommand{\helpedby}{\stackrel{(+)}\longleftarrow}
% \newcommand{\hurtby}{\stackrel{(-)}\longleftarrow}
\newcommand{\helps}{\overset{+}{\longrightarrow}}
\newcommand{\hurts}{\overset{-}{\longrightarrow}}
\newcommand{\helpedby}{\overset{+}{\longleftarrow}}
\newcommand{\hurtby}{\overset{-}{\longleftarrow}}
\newcommand{\entails}{\overset{\oplus}{\longrightarrow}}
\newcommand{\doesnotentail}{\overset{\oplus}{\longleftarrow}}
\newcommand{\relatedby}{\overset{r}{\longrightarrow}}
\newcommand{\ir}{\textsc{ir}\xspace}
\newcommand{\wiqa}{\textsc{wiqa}\xspace}
\newcommand{\quartz}{\textsc{quartz}\xspace}
\newcommand{\quarel}{\textsc{quarel}\xspace}
\newcommand{\defeasible}{\textsc{defeasible}\xspace}
\newcommand{\bert}{\textsc{wiqa-bert}\xspace}
\newcommand{\dotf}{\textsc{dot}\xspace}
\newcommand{\qa}{\textsc{qa}\xspace}
\newcommand{\ours}{\textsc{mercurie}\xspace}  % m explanation reasoning curie
\newcommand{\comet}{\textsc{comet}\xspace}
\newcommand{\plm}{\textsc{plm}\xspace}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\lm}{$\mathcal{L}$\xspace}
\newcommand{\calM}{$\mathcal{M}$\xspace}


\newcommand{\calG}{$\mathcal{G}$\xspace}
\newcommand{\GENS}{$\mathcal{M}^{*}$\xspace}
\newcommand{\GEN}{\calM}
\newcommand{\CORR}{\calG}
\newcommand{\gpt}{\texttt{GPT}\xspace}
\newcommand{\gptt}{\texttt{GPT-2}\xspace}
\newcommand{\tf}{\texttt{T5}\xspace}
\newcommand{\cf}{\textit{cf}\xspace}

\newcommand{\bleu}{\texttt{BLEU}\xspace}
\newcommand{\rouge}{\texttt{ROUGE}\xspace}
\newcommand{\upd}{$\mathbf{S}$\xspace}
\newcommand{\hypo}{$\mathbf{H}$\xspace}
\newcommand{\pre}{$\mathbf{P}$\xspace}
\newcommand{\phu}{$\mathbf{PHS}$\xspace}
\newcommand{\Up}{\textbf{U}\xspace}
\newcommand{\ig}{\textbf{I}\xspace}
\newcommand{\tgen}{\textbf{IGEN}\xspace}
\newcommand{\tgenqa}{\textbf{IGEN-QA}\xspace}
\newcommand{\utype}{\textbf{T}\xspace}
\newcommand{\dquery}{(\pre, \hypo, \upd, \utype)\xspace}

\newcommand{\atomic}{\textsc{atomic}\xspace}
\newcommand{\snli}{\textsc{snli}\xspace}
\newcommand{\social}{\textsc{social}\xspace}
\newcommand{\gengraph}{$\mathbf{G}$\xspace}
\newcommand{\geninfo}{$<$Generated info$>$\xspace}
\newcommand{\sts}{sequence-to-sequence\xspace}
\newcommand{\rqone}{\textsc{rq1}\xspace}
\newcommand{\rqtwo}{\textsc{rq2}\xspace}

\def\@withdot.{\ifmmode\!\string/\!
               \else\kern-1.8pt\string/\kern-1.8pt\fi.}
\newcommand{\inten}{\textit{Intensifies}\xspace}
\newcommand{\atten}{\textit{Attenuates}\xspace}
\newcommand{\dques}{(\pre, \hypo, \upd)\xspace}
\newcommand{\dquesgra}{(\pre, \hypo, \upd, \gengraph)\xspace}
\newcommand{\nle}{\textsc{nl-edit}\xspace}



\newcommand{\squishlist}{
  \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }
\newcommand{\reallysquishlist}{
  \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{0.2em} \setlength{\labelwidth}{0.2em}
      \setlength{\labelsep}{0.2em} } }

 \newcommand{\squishend}{
     \end{list} 
 }

 

==> mercurie/sections-old/feedback.tex <==
\section{Human feedback on $\mathcal{M}$}
\label{sec:feedback-defeasible}





In this section, we propose a method to take feedback on the output of \GEN.

\subsection{Human feedback}



We evaluate the graphs produced by \calM for defeasible reasoning using human evaluators. Two human judges evaluated 100 graphs produced by \calM. 
The judges found that all the graphs had the correct structure, but 70\% of them had \textit{repeated} nodes with the same information.

Each node in an influence graph plays a specific role (e.g., positive contextualizer or mediator). Thus, repeated nodes violate the semantic structure of a graph.
Additionally, they also reduce the amount of information carried by each graph.
For defeasible reasoning, we focus on reducing this repetition of nodes in each graph.
We note that we do not utilize the edge structure of the graph for this work or take feedback on it.
The structure of the graphs is assumed to be fixed.
Our intuition is that reducing the number of repeated nodes will improve the quality of these graphs, making them more useful for downstream tasks.
To be consistent across tasks, we refer to such graphs with repeated nodes as being \textit{incorrect graphs}.


\SetKwInput{KwGiven}{Given}
\SetKwInput{KwInit}{Init}
\begin{algorithm}[!h]
\SetAlgoLined
\KwGiven{Inference graphs G generated by \GEN, and G* generated by \GEN*}
\KwResult{Training data for \CORR}
\KwInit{$\mathcal{D} \gets [ ]$}
\For{$i \gets 1, 2, \ldots, |\mathcal{M}|$}{
$F_{G_i} = feedback(G_i)$ \;
$F_{G_i}* = feedback(G_i*)$\;
\uIf{$F_{G_i} \not = \emptyset$ and $F_{G_i}* = \emptyset$}{
\tcc{$G_i$ has problems, $G_i*$ is good}
$\mathcal{D} = \mathcal{D} \cup (G_i, F_{G_i}, G_i*)$\;
} \uElseIf {$F_G = \emptyset$ and $F_G* = \emptyset$} {
\tcc{Both $G_i$ and $G_i*$ are good}
$\mathcal{D} = \mathcal{D} \cup (G_i, \text{No issues, looks good}, G_i*)$\;
}
}
\KwRet{$\mathcal{D}$}
\caption{Generating training data for \CORR using human feedback.}
\label{alg:alg-train-for-corr}
\end{algorithm}

\subsection{Automating human-like feedback}
\label{sec:automate-human-like-feedback}
We observed that humans found it cognitively challenging to look at multiple nodes and check for the consistency of nodes and repetition of content across multiple unrelated or opposite polarity nodes. In contrast, prior work on assembling structure edit commands relies on the relative simplicity of the structure (such as in an SQL query), allowing targeted feedback. This is not possible in our case, owing to the sizeable cognitive load of manually labeling each node while maintaining structural consistency. Therefore, using human annotations, we devised a simple rule-based system $F$ that uses token-based overlap to detect repetitions while preventing spurious matches due to negation. 
Figures \ref{fig:snliexample}, \ref{fig:atomicexample}, and \ref{fig:socialexample} show examples of various kinds of inconsistencies and the corresponding feedback.


\subsection{Automating expected corrected graph}
\label{sec:automate-expected-corrected-graph}
Ideally, it would be desirable to have training data that provides a \textit{fixed graph} corresponding to each incorrect graph. 
However, we realized that manually fixing incorrect graphs is not scalable, as it requires identifying repeated nodes and then coming up with a label that would remove the repetitions across the graph.
We circumvent this issue by training another version of graph generator \GENS.
The training process of \GENS closely follows that of \GEN: we set the input to $P \Vert H \Vert S \Vert T$ and the output to $G$.
Note that the only difference here from \GEN is that the generation is now additionally conditioned on the edges, leading to more diverse and possibly less noisy graphs.

During inference, we obtain a graph for the defeasible query \phu by setting passage = \pre, hypothesis = \hypo, and situation = \upd, as discussed. Figure~\ref{fig:deftrain} shows the details of the training process.

We further note that such conditioning is not possible for the general case since the graph edges are not available with defeasible queries.

We use T5-11B~\cite{raffel2020exploring} as our graph generator \GEN, feedback graph generator \GENS, as well as graph corrector \CORR.
\begin{figure*}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.80\linewidth]{imgs/snli_bad.pdf}
   \caption{\textit{C-, C+ and S,S- are overlapping.}}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{imgs/social_bad.pdf}
  \caption{\textit{C-,C+,S,S-  and M-, M+, H+ are overlapping.}}
\end{minipage}
  \captionof{figure}{Incorrect graphs generated by \GEN for SNLI (left) SOCIAL domains of Defeasible. The feedback on each graph is mentioned in caption, and we provide the fixed versions of these graphs in the Appendix.}
  \label{fig:feedbackexample}
\end{figure*}

==> mercurie/sections-old/introduction-v1.5.tex <==
\section{Introduction}












% The story.

% \squishlist
% \item Current challenges in Defeasible task (not interpretable, models give reflexive answers -- we might be able to use published error analysis). 
% \item Existing cogsci literature suggests humans form a mental model. This paper primarily investigates whether a machine can benefit from this insight. (we might be able to show that this might hold in principle through an example/analysis from published error analysis).
% \item (+) So we make a new system that can generate high quality inference graphs (better than past models, that we compare with). To do this we included a graph correction module.
% \item (+) We show that with this additional "model" of the question scenario, we can achieve sota on all three datasets related to defeasible reasoning. Past work included these graphs in the question as a string  representation, however we include a module for more meaningful encoding of those graphs than past methods and show that this module is important and helpful too.
% \item (+) Then we discuss the bigger impact of our results - (i) borrowing from cogsci helped on def. inf., (ii) it might help similarly in other tasks if we form a mental model of the question scenario.
% \squishend
% }


% Humans often use background information to respond to a commonsense query.
% Consider a question: \textit{Suppose a contagious respiratory virus is spreading. To avoid getting sick, should one wear a mask in public?} A typical response to this question would be a yes. 
% On the surface, the impact of wearing a mask on avoiding sickness might be obvious.
% However, to holistically reason about this scenario and explain this decision, it becomes important to think about events and facts that helped in reaching the conclusion: wearing a mask does not have a direct effect on the sickness, but it causes less virus to enter the body, thus reducing the chances of getting sick.
% While such \textit{mediating} events are often used instinctively while dealing with commonsense situations, realizing them might help in contextualizing the decision.

Defeasible inference~\cite{rudinger-etal-2020-thinking} is a mode of reasoning in which given a premise \pre (Rob went for a hike), a hypothesis \hypo (Rob saw an elephant, it was pink) may be weakened or overturned in light of new evidence i.e., a situation \upd (Rob often has hallucinations). The non-monotonic nature of this reasoning, makes it a  challenging task~\cite{Morgan2004TheNO}. \citet{rudinger-etal-2020-thinking} show that if the currently best performing pre-trained language model on defeasible inference is asked to generate \upd given \pre and \hypo, then it suffers from two problems: (i) not staying on topic as they often ignore \pre. For instance, when the premise mentions picking up someone at the airport, but the update talks about driving them there. (ii) not drawing meaningful connections between \pre, \hypo, and \upd. For instance, in about 25\% of the predictions, \upd and \hypo or \upd and \pre were found to be repeated.

% NIKET: TEMPORARILY commenting as an alternative 
% \niket{make this paragraph tighter, and introduce notion of premise, hypo, update}
% Humans often use background information to respond to a commonsense query. Consider this scenario: Given a premise \textit{That a person falls to the ground} and a hypothesis that \textit{the person gets hurt}. While an injury can \emph{strengthen} the hypothesis, an update that \emph{the person fell on a soft surface} can \emph{weaken} the initial hypothesis. While humans can instinctively answer these questions and deal with such commonsense situations, it is an open question as to whether machines can benefit through a similar line of reasoning.







% It is natural for a human to answer \emph{yes}, yet a new information like \niket{This happened in a small bedroom.} \textit{The person fell on a soft surface} can weaken the initial answer. Reasoning in such situations would require us to answer two important questions - \emph{Does the new evidence change the original answer ?} and \emph{Why did the original answer change or not change ?}. Defeasible reasoning is this mode of reasoning where a previous conclusion can be strengthened or weakened by a new observation. While humans can instinctively answer these questions and deal with such commonsense situations, it is an open question as to whether machines can benefit through a similar line of reasoning. 



% Such background information plays an especially important role in defeasible reasoning~\cite{rudinger-etal-2020-thinking}, a mode of reasoning that aims to judge the impact of an event~(e.g., wearing masks) on a hypothesis~(e.g., less sickness), in the context of a premise~(e.g., a contagious respiratory virus is spreading).
% \citet{rudinger-etal-2020-thinking} derive a defeasible reasoning dataset~(\defeasible) from three varied phenomenon: commonsense reasoning~\cite{sap2019atomic}, social norms~\cite{forbes2020social}, and natural language inference~\cite{bowman2015large}.
% Each sample in \defeasible consists of an update event \upd, a premise \pre, and a hypothesis \hypo.
% The update \upd either intensifies or attenuates the the hypothesis \hypo.
% The dataset only specifies the type of the type of the update; the reason for the relationship between the update \upd and the hypothesis \hypo is not specified.

A prominent approach in cognitive science literature is to support defeasible reasoning with an \emph{inference graph} \citep{Pollock2009ARS}, which can be seen as a \emph{mental model} of the question scenario before answering the question. Humans find inference graphs helpful in this task (manually \cite{Pollock2009ARS} and automatically constructed \cite{defeasible-human-helps-paper} inference graphs). Inference graphs draw connections between the \pre, \hypo and \upd through mediating events. 
However, current automated methods to defeasible reasoning use an end-to-end approach without first modeling the question scenario, which may hint towards why they deviate from the topic and make repetition errors. This paper asks the natural question whether modeling the question scenario with inference graphs could help machines in defeasible reasoning? 

% part of the paragraph above.
% For defeasible inference task, humans have found it helpful to consult inference graphs (both manually \cite{Pollock2009ARS} and automatically constructed \cite{defeasible-human-helps-paper} inference graphs). Inference graphs draw connections between the \pre, \hypo and \upd through mediating events. 
% However, current automated methods to defeasible reasoning use an end-to-end approach without first modeling the question scenario, which may hint towards why they deviate from the topic and make repetition errors. 




% \cite{rudinger-etal-2020-thinking} show that current pre-trained language models that generate \upd given \pre and \hypo suffer from two problems: (i) not staying on topic by ignoring \pre. For instance, when the premise mentions picking up someone at the airport, but the update talks about driving them there. (ii) and not using drawing a meaningful connection between the hypothesis and premise or (ii) repeating the \hypo or \pre for the 








% NIKET: TEMPORARILY commenting as an alternative 
% Generation approaches for defeasible reasoning using pretrained language models have been shown to suffer from two major limitations - language models often generate strengthening observation instead of a weakening one (or vice-versa) and they often repeat text from input itself \citep{rudinger-etal-2020-thinking}. In this paper, we aim to address these shortcomings by (i) augmenting structured inference graphs to defeasible reasoning tasks and (ii) removing redundancies in such inference graphs leading to improved downstream task performance. 



% this paper investigates whether a machine can also benefit from this insight by (i) proposing a method to create inference graphs without human annotations \am{we should not add this as a contribution}, instead use \cite{defeasible-human-helps-paper} and (ii) whether they help in the downstream defeasible reasoning task. 



\textbf{Proposed system}: Our approach is, given a question, to have a model first create a graph of relevant influences (inference graph from para 2), and then use that graph as an additional input when answering the question. Our proposed system, \ours, comprises of a graph generation module, and a graph encoding module to use the generated graph for QA.

To generate inference graphs, we build upon past work that uses a sequence to sequence approach \cite{defeasible-human-helps-paper}. Their model uses data augmentation to create like-gold graphs. However, the resulting graphs can often be erroneous, and \ours includes an error correction module to generate higher quality inference graphs. This was important because we found that better graphs are more helpful in the QA task.

The generated inference graph is used for the QA task on three existing defeasible inference datasets from diverse domains, viz., $\delta$-SNLI (natural language inference) \cite{bowman2015large}, $\delta$-social (reasoning about social norms) \cite{forbes2020social}, and Atomic (commonsense reasoning) \cite{sap2019atsosomeomic}. We show that by simply augmenting the question with our generated  graphs, there are some gains on all datasets. Importantly, we show that with a more judicious  encoding of the graph augmented question that accounts for interactions between the graph nodes, the QA task accuracy improves substantially across all datasets. To achieve this, we use the mixture of experts approach \cite{mixture-of-experts-paper} to include mixture of experts layers during encoding, enabling the ability to selectively attend to certain nodes while capturing their interactions. 

In summary, our contributions are:
\squishlist
\item We borrow inference graph concept from cognitive science literature to show benefits in defeasible inference QA task. Using an error correction module in the graph generation process, and a judicious encoding of the graph augmented question, \ours achieves a new state-of-the-art over three defeasible datasets. 
\item Our work illustrates that performance can be improved by guiding a system to think about a question. This encourages future studies on other tasks, where the question scenario can be modeled first, rather than answering reflexively. 
\squishend


==> mercurie/sections-old/introduction.tex <==
\section{Introduction}
\am{Algorithm 1 needs to be fixed. Clarify that we don't really take human feedback. Add a running example. Think of a different word for non-actionable, clarify defeasible reasoning by drawing connections with the text entailment.}

\am{Check if the other nodes are changed more for the no feedback case.}

\begin{figure*}[!ht]
\centering
{\includegraphics[scale=0.35]{imgs/pipeline.pdf}}
\caption{Our pipeline: the output generated by \GEN is corrected by \CORR using human feedback.}
\label{fig:pipeline}
\end{figure*}

Interactive Machine Learning allows humans to give feedback to the models, often leading to improved accuracy \citep{Fails2003InteractiveML,Raghavan2006ActiveLW,Settles2011ClosingTL}. Interactive systems for NLP have used human-in-the-loop style interactions for helping refugee settlement \citep{Brown2016DesigningFT}, aligning topic models \citep{Yuan2018MultilingualAI} and enhancing bilingual word embeddings \citep{Yuan2020InteractiveRO}. Neural models have made advancements in explanation generation but are expensive to retrain.
This paper aims to improve the model output through natural language feedback (e.g., on its explanation) without retraining. 

One line of prior approaches (interactive semantic parsing approach) \cite{elgohary2021nl, percy-2016-learning-language-games-interaction-shouldrn} parse natural language user feedback into a set of edit operations, which can then be executed on the incorrect explanation structure, thereby correcting the explanation.
In these approaches, the feedback is specific to a semantic parsing schema and has to be specialized, i.e., directly mapped to specific instructions or literals, limiting its generalizability. 
Moreover, the feedback is expected to be actionable, containing a specific set of edit operations expressed in natural language. However, real-world human feedback is often imprecise and not directly actionable. Another line of prior approaches (interactive reasoning approach)  \citep{Talmor2020TeachingPM} explore interactivity by enriching the context of an input sample through human feedback. However, for the human giving the feedback, the model is a black box -- so the human does not know what the model's internal belief is and how it will change based on the feedback. 

These two lines of prior approaches inspire this paper -- we provide more transparency to the human than the interactive reasoning approach as the model receives feedback on the explanation (similar to the interactive semantic parsing approach). We do this while relaxing the assumptions of the parsing approach -- our feedback does not have a task-specific structure, and it is not assumed to be actionable (similar to the interactive reasoning approach).


We introduce \ours, a pipeline system with two components, a previously trained neural model $\mathcal{M}$ and a graph corrector $\mathcal{G}$. It takes as input any previously trained neural model $\mathcal{M}$ capable of generating an explanation structure. The second input is a natural language human feedback on the generated explanation structure (for example, that some nodes are inconsistent with the rest of the graph). As output, it produces a better explanation structure.
 
% \ours is a pipeline system with two components, firstly $\mathcal{M}$ and then a graph corrector $\mathcal{G}$. 

The contributions of this work are:
\squishlist
\item We demonstrate a system that shows that an explainable NLP model output can be improved through natural feedback on their explanations. Experiments show that \ours can improve the consistency of explanation structures by up to 40\% (\S\ref{sec:feedback-defeasible}).
\item We also show downstream task (defeasible inference \citep{rudinger-etal-2020-thinking}) improvement for all domains by at least 1.2 points on accuracy (\S\ref{sec:results}).
\squishend






\SetKwRepeat{Do}{do}{while}
\SetKwInput{KwGiven}{Given}
\SetKwInput{KwInit}{Init}
\SetKwInput{KwTrainCorr}{Train \CORR on $\mathcal{D}_{\mathcal{G}}$}
\SetKwInput{KwInference}{Inference}
\begin{algorithm}[ht]
\SetAlgoLined
\KwGiven{\GEN: $x \rightarrow  \tilde{y}$, $\{x_i\}_{i=1}^{N}$ } % section 2
\vspace{0.7em}
\KwTrainCorr{}
\Indp
$\mathcal{D}_{\mathcal{G}} = \emptyset$\;
\For{$i \gets 1, 2, \ldots, N$}{
$\tilde{y}_i = \mathcal{M}(x_i)$\;
$I_i = \texttt{feedback}(\tilde{y}_i)$\;  %
$y_i = \texttt{human}(\tilde{y}_i)$\; %section 3
$\mathcal{D}_{\mathcal{G}} = \mathcal{D}_{\mathcal{G}} \cup (x_i, I_i, \tilde{y}_i, y_i)$\;
}

\Indm
\Indp Train \CORR on $(x, I, \tilde{y}) \rightarrow  y$ \;  % section 4
\Indm
\vspace{0.7em}
\KwInference{}  % section 4
\Indp

$\tilde{y} = \mathcal{M}(x)$\;

\While{$I: \texttt{feedback}(\tilde{y}) \neq \emptyset$} {
$\tilde{y} = \mathcal{G}(x, I, \tilde{y})$\;
}
$y = \tilde{y}$\;

\caption{\ours algorithm to correct explanations through human feedback}
\label{alg:alg-1}
\end{algorithm}


% \am{
% \begin{enumerate}
%     \item Defeasible reasoning
%     \item Inference graphs for defeasible reasoning, and refer to the previous work (Show a defeasible query, and a corresponding graph).
%     \item They found that the inference graphs were useful for defeasible reasoning for humans.
%     \item We build upon the work and show that: i) reducing the amount of repetition helps in improving the accuracy, ii) A model that mimics consuming the graph in the way humans did performs better.
% \end{enumerate}
% }


==> mercurie/sections-old/methodology.tex <==
\section{Methodology}
We now evaluate the efficacy of the graphs generated by \GEN and corrected by \CORR on the defeasible inference task.
As mentioned in Section~\ref{sec:task-defeasible}, the goal of the defeasible inference task is to classify an update \upd as a strengthener or weakener of a hypothesis \hypo in the context of premise \pre.

Let $M$ be the graph generated by \GEN for the query \phu.
The graph $M$ and the feedback $F$ on $M$ are then supplied to \CORR to obtain $G$.
We overload the notation and use $M$ and $G$ to refer to the nodes of the graphs generated by \GEN and \CORR, respectively.
Thus, given each defeasible query \phu, we obtain $M$: the set of nodes generated \GEN and $G$: the set of nodes generated by \CORR.


Following \citet{rudinger-etal-2020-thinking}, we prefix a given sequence of tokens $T$ with a special beginning-of-sequence (BOS) token.
$T$ is then encoded using RoBERTa-base~\cite{liu2019roberta}\footnote{We use the implementation by~\cite{wolf2019huggingface}}, and
the hidden representation corresponding to BOS is passed to a classifier (single-layer MLP).
We train three classifiers, each following the above-described architecture with different inputs: (i) Baseline: $T = P \Vert H \Vert S$, (ii) \GEN:  $T = P \Vert H \Vert M \Vert S$, and (iii) \CORR: $T = P \Vert H \Vert G \Vert S$. We report the results in Table~\ref{tab:overall-main-result}, and observe that: (i) Despite the relative simplicity of our approach (concatenating nodes with the query), both \GEN (concatenates noisy graph) and \CORR (concatenates cleaner graph) improve over the baseline. This shows that these explanation structures help enrich the context in the defeasible reasoning task. (ii) \CORR outperforms both the baseline and \GEN, showing that reducing the inconsistencies and repetitions improves end task performance.





==> mercurie/sections-old/results.tex <==
\section{Results}
\label{sec:results}

In this section, we answer two questions: i) Does \CORR reduce the inconsistencies in the graphs? ii) Does using graphs generated by \CORR help the end task?


\subsection{Does \CORR reduce the inconsistencies in the graphs?}


We evaluate the repetitions in the graphs using two metrics:
\squishlist
    \item \textbf{rep. per graph:} the average number of repeated nodes in the graphs produced by \GEN and \CORR.
    \item \textbf{\% with repetitions:} the percentage of graphs with at least one repeated node.
\squishend

As Table~\ref{tab:rq1-main-defeasible} shows, \CORR reduces the average repetitions by 40\% (2.11 to 1.25) and reduces the fraction of graphs with at least one repetition by 25.7 on average.


\begin{table}[!h]
\begin{tabular}{p{0.075\textwidth}p{0.09\textwidth}|p{0.06\textwidth}p{0.06\textwidth}p{0.06\textwidth}}
\toprule
 &  Metric (repetitions) & no feedback (\GEN) & w/ feedback (\CORR) & \CORR w/o feedback \\
\midrule
\atomic & per graph  & 2.05   &  1.26 & \textbf{1.16} \\\cline{2-5}
                           & \% graphs  &  72    &  48 & \textbf{45} \\
\midrule
\snli & per graph   & 2.09   &  1.18 & \textbf{1.14} \\\cline{2-5}
                           & \% graphs &  73 &    46 & \textbf{45}  \\
\midrule
\social & per graph   & 2.2   & 1.32 & \textbf{1.27} \\\cline{2-5}
                          & \% graphs & 75    & 49 & \textbf{48} \\
\midrule
Average & per graph   & 2.11   & 1.25 & \textbf{1.19} \\\cline{2-5}
                          & \% graphs & 73.3    & 47.6 & \textbf{46} \\
\midrule

\end{tabular}
\caption{\CORR reduces the inconsistencies in the graphs. The number of repetitions on average per graph and percentage of graphs with some repetition, both improve.   
}
\label{tab:rq1-main-defeasible}
\end{table}





\subsection{Does using graphs generated by \CORR help the end task?}
\label{sec:rq2}

We now evaluate the efficacy of the graphs generated by \GEN and corrected by \CORR on the defeasible inference task.
As mentioned in Section~\ref{sec:task-defeasible}, the goal of the defeasible inference task is to classify an update \upd as a strengthener or weakener of a hypothesis \hypo in the context of premise \pre.

Let $M$ be the graph generated by \GEN for the query \phu.
The graph $M$ and the feedback $F$ on $M$ are then supplied to \CORR to obtain $G$.
We overload the notation and use $M$ and $G$ to refer to the nodes of the graphs generated by \GEN and \CORR, respectively.
Thus, given each defeasible query \phu, we obtain $M$: the set of nodes generated \GEN and $G$: the set of nodes generated by \CORR.


Following \citet{rudinger-etal-2020-thinking}, we prefix a given sequence of tokens $T$ with a special beginning-of-sequence (BOS) token.
$T$ is then encoded using RoBERTa-base~\cite{liu2019roberta}\footnote{We use the implementation by~\cite{wolf2019huggingface}}, and
the hidden representation corresponding to BOS is passed to a classifier (single-layer MLP).
We train three classifiers, each following the above-described architecture with different inputs: (i) Baseline: $T = P \Vert H \Vert S$, (ii) \GEN:  $T = P \Vert H \Vert M \Vert S$, and (iii) \CORR: $T = P \Vert H \Vert G \Vert S$. We report the results in Table~\ref{tab:rq2-main-defeasible}, and observe that: (i) Despite the relative simplicity of our approach (concatenating nodes with the query), both \GEN (concatenates noisy graph) and \CORR (concatenates cleaner graph) improve over the baseline. This shows that these explanation structures help enrich the context in the defeasible reasoning task. (ii) \CORR outperforms both the baseline and \GEN, showing that reducing the inconsistencies and repetitions improves end task performance.



\begin{table*}[!h]
\centering
\begin{tabular}{lrrrr}
\toprule
        
 & Baseline & \GEN & \CORR & \CORR w/o feedback \\
\midrule
\atomic   & 78.3   & 78.78    & 79.48 & 78.35 \\
\snli    & 81.6   & 82.16    & 83.11  & 83.88  \\
\social  & 86.2   & 86.75    &  87.24 & 87.75  \\
\midrule
average  & 82.03   & 82.56    & 83.27 & 83.32  \\
\bottomrule
\end{tabular}
\caption{Results on Defeasible inference without using graphs (Baseline~\cite{rudinger-etal-2020-thinking}), using graphs generated by \GEN, and graphs corrected with feedback by \CORR. {*} indicates statistical significance}
\label{tab:rq2-main-defeasible}
\end{table*}

\begin{table*}[!h]
\centering
\begin{tabular}{lrrrr}
\toprule
 & \GEN & \CORR & \CORR w/o feedback \\
\midrule
\atomic  & 78.54  & 79.14 & 78.78 \\
\snli & 83.83 &  85.59  & 83.44 \\
\social &  88.23 & 88.62& 88.21  \\
\midrule
average & 83.53 & 84.5 & 83.48  \\
\bottomrule
\end{tabular}
\caption{MOE (v0)}
\label{tab:rq3-main-defeasible}
\end{table*}

\begin{table*}[!h]
\centering
\begin{tabular}{lrrrr}
\toprule
 & \GEN & \CORR & \CORR w/o feedback \\
\midrule
\atomic  & 78.83  & 79.19 & 79.34 \\
\snli & 82 &  83.09  & 83.93 \\
\social &  88.44 & 88.44 & 88.47  \\
\midrule
average & 83.09 & 83.57 & 83.91  \\
\bottomrule
\end{tabular}
\caption{MOE (sa)}
\label{tab:rq3-main-defeasible}
\end{table*}

\begin{table*}[!h]
\centering
\begin{tabular}{lrrrr}
\toprule
 & \GEN & \CORR & \CORR w/o feedback \\
\midrule
\atomic  & 78.25     & 78.85 & 78.9 \\
\snli     &   82.63  & 82.36 & 83.56  \\
\social   &  87.92   & 88.12 & 88.08  \\
\midrule
average   & 82.93   & 83.11 & 83.51  \\
\bottomrule
\end{tabular}
\caption{GCN}
\label{tab:rq4-main-defeasible}
\end{table*}



\newpage

\begin{table}[!h]
\centering
\begin{tabular}{lrrrr}
\toprule
 & \atomic & \snli & \social \\
\midrule
\small{Prev-SOTA}   & 78.3  & 81.6 & 86.2  \\
\ours &   \textbf{79.1}  & \textbf{85.6} & \textbf{88.6}  \\
\bottomrule
\end{tabular}
\caption{This table shows that \ours is better on multiple domains on two tasks defeasible inference and procedural understanding. Demonstrates  self-thinking on ques through generating an inference gr. helps.}
\label{tab:overall-main-result}
\end{table}


\subsection{Reasons behind these gains}

\squishlist
\item \textbf{graph quality: good graphs, better output?}
\item \textbf{graph repr.: best way to consume graph?}
\item \textbf{self-introspection: does feedback help?}
\squishend


\subsection{Error analysis}

\squishlist
\item \textbf{When graphs hurt} show examples...
\item \textbf{When good graphs cannot be used} show ex...
\item \textbf{When graphs are bad} show examples...
\squishend

\newpage


==> mercurie/sections-old/rq1.tex <==
\section{Correcting explanation structure through human feedback}
\label{sec:rq1}

\am{Here, suggest some additional ways of creating the feedback}
\am{Need to add the without feedback baseline}

\begin{figure*}[!htb]
\minipage{0.33\textwidth}
  \includegraphics[width=\linewidth]{imgs/end_to_end_gen.pdf}
\endminipage\hfill
\minipage{0.33\textwidth}
  \includegraphics[width=\linewidth]{imgs/end_to_end_genstar.pdf}
\endminipage\hfill
\minipage{0.33\textwidth}%
  \includegraphics[width=\linewidth]{imgs/end_to_end_corr.pdf}
\endminipage
\caption{The graphs generated by \GEN (left), \GENS (middle), and \CORR (right).The input graph has repetitions for nodes $\{C{-}, S{-}\}$,  $\{C{+}, H{+}\}$, and $\{M{-}, M{+}\}$. The corrected graph replaces the repetitions with meaningful labels.}
\label{fig:defeasible_incorrect}
\end{figure*}


Can we make use of the feedback described \S \ref{sec:feedback-defeasible}? We show that we can train a model, \CORR, that takes that feedback and improves \GEN. That is, given \phu, \GEN generates a potentially noisy graph (\S \ref{sec:gen-for-defeasible}) - and \CORR learns to correct this graph using the automatic human-like feedback (\S \ref{sec:automate-human-like-feedback}) and compute loss over the expected corrected graph (\S \ref{sec:automate-expected-corrected-graph}). First, we show this graph correction system \CORR, followed by empirically measuring the effectiveness of \CORR.


\subsection{Training the graph corrector \CORR}
We now proceed to train the graph corrector \CORR using Algorithm~\ref{alg:alg-train-for-corr}. 
The \CORR is also trained as a sequence-to-sequence model.
For a given query \phu, the graphs generated by \GEN and \GENS are first paired.
From these pairs, we only retain those cases where the \GEN graph is incorrect, whereas \GENS graph is not, as identified by our rule-based feedback system $F$.
We record each such example as $(G', F(G'), G*)$.
We also retain pairs where both $G'$ and $G''$ are correct, and in those cases, the feedback $F(G')$ is set to \textit{no issues, looks good}.
This is then fed to our generation model, which is trained to generate $G^{*}$ from $G', F(G')$.



Training \CORR completes our pipeline for obtaining high-quality graphs for each defeasible query.
First, given a defeasible query \phu, we generate a potentially incorrect graph. 
G' using \GEN.
We then use the feedback generator $F$ to obtain feedback $F(G')$ on $G'$.
The tuple $(G', F(G'))$ is then fed to \CORR to obtain a corrected graph G.


==> mercurie/sections-old/task_dataset-v-1.5.tex <==
\section{Task and Dataset}
% \am{
% \begin{enumerate}
%     \item Defeasible inference
%     \item Graphs for defeasible inference
% \end{enumerate}
% }



\subsection{Datasets}
\begin{table}[!h]
\small
\centering
%  \resizebox{\columnwidth}{!}{
\begin{tabular}{llrr}
\toprule
Dataset & Split & \# Samples & Total\\ \midrule
 \multirow{3}{*}{\wiqa} & train & 1522 & \multirow{3}{*}{2107} \\
      & test   & 189  \\
& dev  & 152 \\ \midrule
 \multirow{3}{*}{\atomic} & train & 35,001 & \multirow{3}{*}{42,977} \\
      & test   & 4137  \\
& dev  & 3839 \\ \midrule
 \multirow{3}{*}{\social} & train & 88,675 & \multirow{3}{*}{92,295} \\
      & test   & 1836  \\
& dev  & 1784 \\ \midrule
 \multirow{3}{*}{\snli} & train & 77,015 & \multirow{3}{*}{95,795} \\
      & test   & 9438  \\
& dev  & 9342 \\
\bottomrule
\end{tabular}
% }
\caption{Number of samples in each dataset by split. \dheeraj{move this detail to footnote} \atomic, \snli, \social are available at~\url{https://github.com/rudinger/defeasible-nli}, \wiqa is available at~\url{https://allenai.org/data/wiqa} . \niket{instead of \wiqa, describe dataset in human helps paper}}
\label{table:data-split}
\end{table}


% \niket{Talk about the domains of defeasible, and clarify that \social has no context.}
% Given the central role that the \wiqa dataset plays in our work, we provide a brief description next.




% \subsubsection{\wiqa}
% \wiqa comprises of 2107 pairs of $(P, G)$ where $P$ is a paragraph that describes a process (e.g., the spread of a virus).
% The inference graph $G$ corresponding to $P$ is a directed acyclic graph (\textsc{dag}) that captures the interactions between the events and their inferences within the context of the process described by $P$. 
% Let $G=(V, E)$, where $V$ denotes the set of vertices and $E$ the set of edges.
% The nodes $n \in V$ are events relevant to the process.
% Each node $n$ is described by a sequence of text tokens.
% The edge set $E$ contains two types of edges: $\textit{helps}$ and $\textit{hurts}$, denoted by \green{green} and \red{red} arrows respectively.
% A $\textit{helps}$ edge between a source node $n_c$ and a target node $n_e$ signifies that the source event $n_c$ positively inferences the target event $n_e$ and a $\textit{hurts}$ edge stands for $n_c$ negatively influencing $n_e$.
% Figure~\ref{fig:virusinferencegraph} shows an example inference graph for the process of ``spread of a virus during a pandemic.''

\begin{figure}[!ht]
\centering
{\includegraphics[scale=0.33]{imgs/igraph_waves.pdf}}
\caption{A sample inference graph for the running example.}
\label{fig:virusinferencegraph}
\end{figure}


\subsubsection{Dataset and Model for graph generation module}
Model and dataset are taken from \cite{defeasible-human-helps-paper}. \niket{write in brief about (human helps) model M that can generate an inference graph; and for training that model they used a dataset that was created and released by that paper. We make use of model M, and our objective is then to make use of M through graph correction module and graph encoding module...}

% In the absence of a large repository of inference graphs for defeasible queries, we propose their automatic generation by learning from \wiqa~\cite{tandon2019wiqa} - a repository of graphs that are similar to an inference graph ( Section~\ref{sec:inferenceinferencemapping}). 
% The main challenge in learning from these graphs is that they are narrowly focused on the procedural text domain. In contrast, defeasible inference task has a wide scope-- thus requiring the transfer technique that we present in \ref{sec:gen-for-defeasible}.

\subsubsection{Dataset for graph correction}
\niket{write about bad graph to good graph}



\subsubsection{Dataset for end task}
We use the $\delta$-\snli, $\delta$-\social, $\delta$-\atomic ... whose size and statistics is mentioned in Table \ref{table:data-split} ...

\niket{how will this dataset be used, mention}

% \subsubsection{Inference graphs for defeasible reasoning}
% \label{sec:inferenceinferencemapping}
% \am{Add citation to the ACL paper, describe how those graphs were used}
% We show that the nodes of an inference graph in \wiqa are similar to the inference graph for defeasible reasoning proposed in ~\cite{Pollock2009ARS}, by showing a semantic mapping between the components of a defeasible query and an inference graph.

% \squishlist
%     \item The premise of a defeasible query \pre and the passage in \wiqa both play a similar role of providing more context for the inference graph.
%     \item Each \wiqa graph has two hypothesis nodes, which capture either the strengthening or weakening of a hypothesis.
%     Thus, there is a natural correspondence between the hypothesis nodes in \wiqa and the hypothesis in defeasible.
%     \item Each inference graph consists of a node $S$, which contains an event grounded in $P$ that signifies a change. This is similar to the update \upd in the defeasible query.
%     % \item Answer \utype $\Leftrightarrow$ $E$: The edge structure of an inference graph remains fixed from $M$ and above. The four edges between $M$ and $H$ nodes take one of the two forms, depending on the nature of the inference of $S$ on $H+$. 
%     % This is also precisely the nature of inference that the situation \upd has on the hypothesis. 
%     % For instance, if \upd weakens \hypo in the context of \pre, the answer \utype will be \textit{weakens}, and the edge between $M+$ and $H-$ will be \red{hurts}.  
% \squishend


% \subsection{Designing \GEN for Defeasible Reasoning}
% \label{sec:gen-for-defeasible}
% Given these similarities, we train a graph-generator on \wiqa and transfer it for defeasible reasoning.
% Our goal is to supplement each defeasible query \phu with an inference graph. We first train a graph generator \calM using \wiqa.
% As discussed, each example in \wiqa consists of a $(P, G)$ pair, where $P$ is the passage, and $G$ is the inference graph.
% We extract the hypothesis node $H$ and the situation node $S$ from $G$ (using the last two nodes in Figure~\ref{fig:virusinferencegraph}). 
% We then train a sequence-to-sequence generation model (based on T5-11B), where the input is the string $P \Vert H \Vert S$ and the output is the corresponding inference graph $G$ encoded as a string.
% During inference, we obtain a graph for the defeasible query \phu by setting passage = \pre, hypothesis = \hypo, and situation = \upd, as discussed. Figure~\ref{fig:deftrain} shows the details of the training process.




==> mercurie/sections-old/task_dataset.tex <==
\section{Task and Dataset}
\label{sec:task-defeasible}

We focus on the task of generating graphs for defeasible inference queries. After presenting the task, we describe the graph generator \GEN that generates an inference graph for a defeasible inference query. Subsequently, we will use the feedback described in \S \ref{sec:feedback-defeasible} to train \CORR, a system that fixes the output generated by \GEN.

\subsection{Task: Defeasible Inference}

Defeasible inference~\cite{rudinger-etal-2020-thinking} is a mode of reasoning in which given a premise \pre, a hypothesis \hypo may be strengthened or weakened in light of new evidence.
For example, given a premise \textit{ocean causes erosion}, the hypothesis \textit{rocks become smaller} will be strengthened by the situation \textit{waves are bigger}, and weakened by the situation \upd \textit{no waves}.
We use \phu to refer to a defeasible query and \utype to the answer~(strengthened or weakened). 

This problem has been widely studied in cognitive science by supporting defeasible inference through argumentative frameworks \cite{Pollock1987DefeasibleR}. Humans have found argumentations helpful in defeasible reasoning, and this insight has led to models that simulate argumentations through an \emph{inference graph}, e.g., \citet{Pollock2009ARS} supplement defeasible queries \phu with an \textit{inference graph}. An inference graph contains events as nodes and the causal relationship between the nodes as edges. The motivation behind using inference graphs is to provide additional context for each \phu query that might help the humans understand the nature of the effect that an update situation \upd has on the hypothesis. Being costly to construct by hand, inference graphs have only been studied at a small scale. 

In the absence of a large repository of inference graphs for defeasible queries, we propose their automatic generation by learning from \wiqa~\cite{tandon2019wiqa} - a repository of graphs that are similar to an inference graph ( Section~\ref{sec:inferenceinfluencemapping}). 
The main challenge in learning from these graphs is that they are narrowly focused on the procedural text domain. In contrast, defeasible inference task has a wide scope-- thus requiring the transfer technique that we present in \ref{sec:gen-for-defeasible}.
Given the central role that the \wiqa dataset plays in our work, we provide a brief description next.




\subsubsection{\wiqa}
\wiqa comprises of 2107 pairs of $(P, G)$ where $P$ is a paragraph that describes a process (e.g., the spread of a virus).
The influence graph $G$ corresponding to $P$ is a directed acyclic graph (\textsc{dag}) that captures the interactions between the events and their influences within the context of the process described by $P$. 
Let $G=(V, E)$, where $V$ denotes the set of vertices and $E$ the set of edges.
The nodes $n \in V$ are events relevant to the process.
Each node $n$ is described by a sequence of text tokens.
The edge set $E$ contains two types of edges: $\textit{helps}$ and $\textit{hurts}$, denoted by \green{green} and \red{red} arrows respectively.
A $\textit{helps}$ edge between a source node $n_c$ and a target node $n_e$ signifies that the source event $n_c$ positively influences the target event $n_e$ and a $\textit{hurts}$ edge stands for $n_c$ negatively influencing $n_e$.
Figure~\ref{fig:virusinfluencegraph} shows an example influence graph for the process of ``spread of a virus during a pandemic.''

\begin{figure}[!ht]
\centering
{\includegraphics[scale=0.38]{imgs/igraph_waves.pdf}}
\caption{A sample influence graph about spread of a virus during a pandemic}
\label{fig:virusinfluencegraph}
\end{figure}

\subsubsection{\wiqa as a repository of inference graphs}
\label{sec:inferenceinfluencemapping}
We show that the nodes of an influence graph in \wiqa are similar to the inference graph for defeasible reasoning proposed in ~\cite{Pollock2009ARS}, by showing a semantic mapping between the components of a defeasible query and an influence graph.

\squishlist
    \item The premise of a defeasible query \pre and the passage in \wiqa both play a similar role of providing more context for the influence graph.
    \item Each \wiqa graph has two hypothesis nodes, which capture either the strengthening or weakening of a hypothesis.
    Thus, there is a natural correspondence between the hypothesis nodes in \wiqa and the hypothesis in defeasible.
    \item Each influence graph consists of a node $S$, which contains an event grounded in $P$ that signifies a change. This is similar to the update \upd in the defeasible query.
    % \item Answer \utype $\Leftrightarrow$ $E$: The edge structure of an influence graph remains fixed from $M$ and above. The four edges between $M$ and $H$ nodes take one of the two forms, depending on the nature of the influence of $S$ on $H+$. 
    % This is also precisely the nature of influence that the situation \upd has on the hypothesis. 
    % For instance, if \upd weakens \hypo in the context of \pre, the answer \utype will be \textit{weakens}, and the edge between $M+$ and $H-$ will be \red{hurts}.  
\squishend


\subsection{Designing \GEN for Defeasible Reasoning}
\label{sec:gen-for-defeasible}
Given these similarities, we train a graph-generator on \wiqa and transfer it for defeasible reasoning.
Our goal is to supplement each defeasible query \phu with an inference graph. We first train a graph generator \calM using \wiqa.
As discussed, each example in \wiqa consists of a $(P, G)$ pair, where $P$ is the passage, and $G$ is the influence graph.
We extract the hypothesis node $H$ and the situation node $S$ from $G$ (using the last two nodes in Figure~\ref{fig:virusinfluencegraph}). 
We then train a sequence-to-sequence generation model (based on T5-11B), where the input is the string $P \Vert H \Vert S$ and the output is the corresponding influence graph $G$ encoded as a string.
During inference, we obtain a graph for the defeasible query \phu by setting passage = \pre, hypothesis = \hypo, and situation = \upd, as discussed. Figure~\ref{fig:deftrain} shows the details of the training process.

\begin{figure*}[!ht]
\centering
{\includegraphics[width=0.90\textwidth,height=0.17\textheight]{imgs/defeasible_m.pdf}}
\caption{Training the graph generator $\mathcal{M}$ for defeasible reasoning.}
\label{fig:deftrain}
\end{figure*}



==> mercurie/sections-without-graphgen/abstract.tex <==
\begin{abstract}
Defeasible reasoning is the mode of reasoning where conclusions can be overturned by taking into account new evidence. Existing cognitive science literature on defeasible reasoning suggests that a person forms a ``mental model'' of the scenario before answering it. Our research goal asks whether neural models can similarly benefit from envisioning the question scenario before answering a defeasible query. Our approach is, given a question, to have a model first create a graph of relevant influences, and then effectively leverage that graph as an additional input when answering the question. We find that \ours achieves a new state-of-the-art on three different defeasible reasoning datasets, as well as now producing justifications for its answers. This result is significant as it illustrates that performance can be improved by guiding a system to ``think about'' a question and explicitly model the scenario, rather than answering reflexively.



% Question-answering (QA) often involves reasoning about {\it chains of influence}. For example, to answer "Can storms increase beach erosion?" a person might reason
% that storms produce bigger waves, resulting in more erosion (hence "yes"). From a cognitive science perspective, a person appears to form a ``mental model''
% of the scenario behind the question before answering it.
% Our research goal asks whether neural models can similarly benefit from envisioning the QA scenario before answering a question. Our approach is, given a question, to have a model first create a graph of relevant influences,
% and then effectively leverage that graph as an additional input when answering the question. We find that \ours achieves a new state-of-the-art on three different defeasible reasoning datasets, as well as now producing justifications for its answers. This result is significant as it suggests model performance in other contexts may similarly be improved by guiding them to ``think about'' a question and explicitly model the scenario, rather than answering reflexively.
\end{abstract}


==> mercurie/sections-without-graphgen/analysis.tex <==
\section{Error analysis}
\label{sec:analysis}
\begin{table}[!ht]
\noindent
% \renewcommand\arraystretch{1.5}
\setlength\tabcolsep{0pt}
\begin{tabular}{c >{\bfseries}r @{\hspace{0.7em}}c @{\hspace{0.4em}}c}
  \multirow{10}{*}{\parbox{1.1cm}{\bfseries\raggedleft}} & 
    & \multicolumn{2}{c}{\bfseries} \\
  & & \bfseries now fail & \bfseries now succ  \\
  & prev fail & \ABox{\scriptsize{\atomic} \small{615}}{\scriptsize{\snli} \small{197} \\ \scriptsize{\social} \small{772}} & \ABox{\scriptsize{\atomic} \small{294}}{\scriptsize{\snli} \small{124} \\ \scriptsize{\social} \small{398}} \\[2.4em] 
  & prev succ & \ABox{\scriptsize{\atomic} \small{207}}{\scriptsize{\snli} \small{68} \\ \scriptsize{\social} \small{302}} & 
  \ABox{\scriptsize{\atomic} \small{3022}}{\scriptsize{\snli} \small{1448} \\ \scriptsize{\social} \small{7967}}  \\
%   & total & P & N 
\end{tabular}
\caption{Confusion matrix on the test split of the three datasets. The differences are highly significant with p-values of $1.1e-04$ on \atomic, $6.5e-05$ on \snli, and $3.2e-04$ on \social using McNemar's test.}
\label{tab:confusion-matrix}
\end{table}
% latex idea from https://tex.stackexchange.com/questions/20267/how-to-construct-a-confusion-matrix-in-latex\textbf{}


Table \ref{tab:confusion-matrix} shows that \ours is able to correct several previously wrong examples. We observe that when \ours corrected previously failing cases, the \nodemoe relied more on mediators, as the average mediator probabilities go up from 0.09 to 0.13 averaged over the datasets. \ours still fails, and more concerning are the cases when previously the model succeeded, and with the appended graph \ours fails. To study this, we annotate 50 random dev samples in total over all three datasets. For each sample, a human marked annotated the errors in the graph, if any. We observe the following error categories\footnote{For more examples see Appendix  Table~\ref{tab:error-analysis-examples})}:
\squishlist
\item \textbf{All nodes off topic (4\%)}: The graph nodes were not on topic. This rarely happens when \ours is unable to distinguish the sense of a word in the input question. For instance, \upd = there is a water fountain in the center -- \ours generated based on an incorrect sense of natural water spring. Another instance, \upd = personX's toy is a car -- \ours generated a real car related graph. 
\item \textbf{Repeated nodes (20\%)}: These may be exact or near-exact matches. Node pairs with similar effects, tend to be repeated in some samples. e.g. S- node is often repeated with contextualizer C- perhaps because these nodes indirectly affect graph nodes in a similar way. 
\item \textbf{Mediators are uninformative (34\%)}: The mediating nodes are not correct or informative. One source of these errors is when the \hypo and \upd are nearly connected by single hop e.g., \hypo = personx pees, and \upd = personx drank a lot of water previously.
\item \textbf{Good graphs are ineffective (42\%)}: These graphs contained the information required to answer the question, but the gating MOE mostly ignored this graph. This could be attributed in part to the observation in histogram in Figure \ref{fig:graphquesmoedist}, that samples with weakener label disproportionately ignore the graph.
\squishend
% from sheet: https://docs.google.com/spreadsheets/d/1EBRFvFlLF2YkTNRTpZZ0xV8SqWST_oAa_LsfOo4kY74/edit#gid=0

The maximum percentage of errors were in \atomic , in part due to low question quality, this is in accordance with the dataset quality results in the original paper.  \cite{rudinger-etal-2020-thinking}.




==> mercurie/sections-without-graphgen/approach.tex <==
\begin{figure}[!ht]
\centering
{\includegraphics[scale=0.27]{mercurie/imgs/example-glass.png}}
\caption{A sample inference graph for the running example.}
\label{fig:igraphexample}
\end{figure}



\section{\ours}



\subsection{Task: Defeasible Inference}
\label{sec:task-defeasible}
Defeasible inference~\cite{rudinger-etal-2020-thinking} is a mode of reasoning in which given a premise \pre, a hypothesis \hypo may be strengthened or weakened in light of new evidence \upd.
For example, given a premise \textit{The drinking glass fell}, the hypothesis \textit{The glass broke} will be weakened by the situation \textit{the glass fell on the pillow}, and strengthened by the situation \upd \textit{the glass fell on the rocks}. We define the input \x=(\pre,\hypo,\upd) and output $\V{y} \in \{strengthens, weakens\}$.

Prior research in psychology~\cite{Pollock2009ARS} and NLP~\cite{defeasible-human-helps-paper} has found that inference graphs can greatly aid human performance at defeasible inference. Inference graph capture the mediating events and the context to facilitate critical thinking, acting as a mental model of the scenario posed by the defeasible query. A sample inference graph is shown in Figure~\ref{fig:igraphexample}.

We answer the question whether neural models can benefit from envisioning the question scenario using an inference graph before answering a defeasible inference query. 




\paragraph{Inference graphs} As inference graphs are central to our work, we give a brief description of their structure next.
Inference graphs were introduced in philosophy by \citet{Pollock2009ARS} to aid defeasible reasoning for humans, and in NLP by \citet{tandon2019wiqa} for a counterfactual reasoning task.


Inference graphs have four kinds of nodes~\cite{Pollock2009ARS,tandon2019wiqa,defeasible-human-helps-paper}: 
\squishlist
\item[i.] \textbf{Contextualizers (C):} these nodes set the context around a situation and connect to the \pre in some way.
\item[ii.] \textbf{Situations (S):} these nodes are new situations that emerge which might overturn an inference.
\item[iii.] \textbf{Hypothesis (H):} Hypothesis nodes describes the outcome/conclusion of the situation.
\item[iv.] \textbf{Mediators (M):} Mediators are nodes that help bridge the knowledge gap between a situation and a hypothesis node by explaining their connection explicitly. These node can either act as a \emph{weakener} or \emph{strengthener}.
\squishend


\paragraph{Dataset of inference graphs for defeasible reasoning} Recently, \cite{madaan2021improving} proposed a sequence-to-sequence approach for obtaining higher-quality graphs for each defeasible query.
They release two datasets: i) a noisy version of the graphs (\mnoisy), and ii) a cleaner version (\mclean).
This gives for each defeasible query \x, an inference graph $\V{G}_\V{x}(\V{V}, \V{E})$ that provides additional context for the query.
We use these graphs in this work.
% \dheeraj{such that the generated graphs provides a rich explanation structure for each defeasible query? motivate why graphs again}.

% Having described our task, we next give an overview of the graph generator \GEN that generates an inference graph for a defeasible inference query. 
% Subsequently, we will use the feedback described in \secref{sec:feedback-defeasible} to train \CORR, a system that fixes the output generated by \GEN.

% \subsection{Overview of \ours}
% The \ours system comprises of two components, (i) Graph generator \GEN, (ii) Graph encoder. \GEN generates an inference graph from the input $x$. We borrow the sequence to sequence approach of \GEN from \citet{defeasible-human-helps-paper} without any changes, and we will describe it very briefly. The inference graphs are then judiciously encoded using the graph encoder, which is our modeling contribution.


% We describe ours as a pipeline...

% - we use the system described in \citet{defeasible-human-helps-paper} 
% - describe the system in a line or two 
% - uses WIQA for transfer learning and it is zero-shot and uses the inference graph structure from WIQA
% - Then each datapoint in defeasible is augmented with the graphs 
% - But the graphs are noisy

% \subsection{Graph generation module}
% Recently, \cite{madaan2021improving} proposed a sequence-to-sequence approach for obtaining higher-quality graphs for each defeasible query.
% They release two datasets: i) a noisy version of the graphs with a high number of repetitions (\mnoisy), and ii) a cleaner version with lesser repetitions (\mclean).
% We use the sequence to sequence approach of \GEN from \citet{madaan2021improving} without any changes to generate inference graph for \x.
% Briefly, their method does \niket{xxxx}
% Using their method, we are able to generate an inference graph given \x\footnote{This dataset was publicly released by the authors at \url{https://tinyurl.com/mercurie}}.


\subsection{Graph augmented defeasible reasoning}
\begin{figure*}
\centering
{\includegraphics[width=0.93\textwidth,height=0.25\textheight]{imgs/moe.pdf}}
\caption{An overview of our method to perform graph-augmented defeasible reasoning using a hierarchical mixture of experts. First, \nodemoe selectively pools the node representations to generate a graph representation \hg. Then, \graphmoe pools the query representation \hq and the graph representation generated by \nodemoe to pass to the upstream classifier.  \niket{make premise gray to distinguish from the remaining nodes which are white.}}
\label{fig:moe}
\end{figure*}
% \niket{First describe the top level augmentation technique, and specific model.}
% \subsubsection{Preliminaries}
% We are given a defeasible query \dques, where the goal is to evaluate affect of an update event \upd on a hypothesis \hypo as \textit{strengthener} or \textit{weakener} in the context of a premise \pre(~\secref{sec:task-defeasible}). 
% \dheeraj{In this section, the task is to (i) encode the graph (ii) encode text and predict the classes (what classes) - make it formal and task setup clear}

Following \citet{rudinger-etal-2020-thinking}, we first concatenate the components \dques of the defeasible query into a single sequence of tokens $\V{x} = (\mathbf{P} \| \mathbf{H} \| \mathbf{S})$, where $\|$ denotes concatenation.
Thus, each sample for our graph-augmented binary-classification task takes the form $((\V{x}, \V{G}), \V{y})$, where  $\V{y} \in \{\text {\textit{strengthener}, \textit{weakener}}\}$.


\paragraph{Outline:} We first use a language model \lm to obtain a dense representation \hq for the defeasible query, and a dense representation \hv for each node $\V{v} \in \V{G}$. The node representations \hv are then pooled using a hierarchical mixture-of-experts (\moe) to obtain a graph representation \hg.
The query representation \hq and the graph representation \hg are combined to solve the defeasible task.
Next, we provide details on obtaining \hq, \hv, and \hg.


%\dheeraj{Describe the role of an encoder and a generic notation here.. }



\subsubsection{Encoding query and nodes}

Let \lm be a pre-trained language model (in our case \roberta~\cite{liu2019roberta}).
We use $\V{h}_{\V{S}} = \mathcal{L}(\V{S}) \in \real{d}$ to denote the dense representation of sequence of tokens $\V{S}$ returned by the language model \lm.
% We interchangeably refer to $\mathcal{L}(\V{S})$ as the encoding of sequence $\V{S}$.
In our case, we use the pooled encoding on the \roberta~encoder - \texttt{<s>} as the sequence representation. 
% A popular design choice for performing such encoding involves running self-attention over $\texttt{[CLS]} \| \V{S}$, and then using the hidden representation corresponding to the special \texttt{[CLS]} token.
% ($\real{n}$) of the first token of the last layer  as $\V{h}_\V{S}$.
% Here, \texttt{[CLS]} is a special token reserved for sequence encoding. 
% Other options include pooling the last hidden layer and using projections.

% \subsection{Method}



% \dheeraj{\paragraph{Query Encoder:}}
% \dheeraj{My suggestion is to keep this paragraph short and brief by saying that we take the pooled [CLS] representation from a PLM (of choice). I dont think we need to add much details here, its pretty clear.}

% \st{\paragraph{Model sketch}}
% \dheeraj{\paragraph{Mixture of Experts Graph Encoder}} 

% \dheeraj{Suggestion: only talk about mixture of experts. GCN things should go straight to baselines for graph encoder in experiments.}

% \dheeraj{start with refering to the figure here.. show how representations of nodes are encoded and how MoE is used... and then summarize in the algorithm} 
% \dheeraj{Also, I dont see the need for an algorithm here, mainy because there is no iteration to understand. Its a fixed setting with few steps, algo seems redundant.}


We encode the defeasible query $\V{x}$ and the nodes of the graph using \lm. Query representation is computed as follows: $\V{h}_\V{x} = \C{L}(\V{x})$. 
%We encode graph \gengraph in two steps, closely following the methodology followed by 
We similarly obtain a matrix of node representations $\nodeset$ by encoding each node $\V{v}$ in \gengraph with \lm as follows: 
\begin{align}
    \V{h}_{\V{V}} = [\V{h}_{v_1}; \V{h}_{v_2}; \ldots; \V{h}_{|\V{V}|}]
    \label{eqn:encode_nodes}
\end{align}


where $\V{h}_{v_i} \in \real{d}$ refers to the dense representation for the $i^{th}$ node of $\V{G}$ derived from \lm (i.e., $\V{h}_{v_i} = \C{L}(v_i)$), and $\V{h}_{\V{V}} \in \real{|\V{V}| \times d}$ to refer to the matrix of node representations.

\subsubsection{Learning graph representations using Mixture-of-experts}
\label{sec:moe_pooling}

% The problem of learning meaningful graph-representations has recently gained a lot of popularity.
% Popular methods typically use graph convolutional networks~\cite{lin2019kagnet} and graph attention to first refine node features, and then use attention to over the nodes to learn a single representation for the graph~\cite{lv2020graph}.

Recently, mixture-of-experts~\cite{jacobs1991adaptive,shazeer2017outrageously,fedus2021switch} has emerged as a promising method of combining multiple feature types.
Mixture-of-experts (\moe) are especially useful when the input consists of multiple \textit{facets}, where each facet has a certain semantic meaning.
Previously, \citet{gu2018universal,chen2019multi} have used the ability of \moe to pool disparate features on low-resource and cross-lingual language tasks.
Since each node in the inference graphs used by us plays a certain role in defeasible reasoning (contextualizer, situation node, mediator etc.), 
we take inspiration from these works to design a hierarchical \moe model to pool node representations $\nodeset$ into a graph representation \hg.

An \moe consists of $n$ expert networks $\V{E_1}, \V{E_2}, \ldots, \V{E_n}$ and a gating network $\V{M}$.
Given an input $\V{x} \in \real{d}$, each expert network $\V{E_i}: \real{d} \rightarrow \real{k}$ learns a transform over the input.
The gating network $\V{M}: \real{d} \rightarrow \Delta^d$ gives the weights $\V{p} = \{p_1, p_2, \ldots, p_n\}$ for combining the expert outputs for the input $\V{x}$.
Finally, the output $\V{y}$ is returned as a convex combination of the expert outputs:

\begin{align}
    \V{p} &= \V{M}(\V{x}) \nonumber \\
     \V{y} &= \sum_{i=1}^{n} p_i \V{E_i(x)}
    \label{eqn:moe}
\end{align}

The output $\V{y}$ can either be the logits for an end task~\cite{shazeer2017outrageously,fedus2021switch} or pooled features that are passed to a downstream learner~\cite{chen2019multi,gu2018universal}.
The gating network $\V{M}$ and the expert networks $\V{E_1}, \V{E_2}, \ldots, \V{E_n}$ are trained end-to-end.
During learning, the gradients to $\V{M}$ help it in learning to correctly mix the output of the experts, by generating a distribution over the experts that favors the best expert for the given input.


\paragraph{Designing hierarchical \moe for defeasible reasoning}

Different parts of the inference graphs might be useful for answering a query to a different degree.
Further, for certain queries graphs might not be useful or distracting and model could rely primarily on the input query alone~\cite{defeasible-human-helps-paper}.
This motivates a need for two-levels architecture that has: (i) the ability to select a subset of the nodes in the graph, and ii) the ability to jointly reason on the query and the graph to varying degrees.

% These requirements, combined with inductive bias of selectively picking input offered by \moe motivate them as the natural choice for pooling graph representation.
Given these requirements, a hierarchical \moe model presents itself as a natural choice to model this task~\ref{fig:moe}.
% Specifically, we employ this hierarchical \moe setup to perform such \textit{selective data augmentation}~(Figure~\ref{fig:moe}).
The first expert (\nodemoe) creates a graph representation by taking a convex-combination of the node representations.
% Following~\cite{defeasible-human-helps-paper}, we do not use edge labels and treat all the graphs as undirected graphs.
The second expert (\graphmoe) then takes a convex-combination of the graph representation returned by \nodemoe and query representation, and passes it to an MLP for the downstream task.


\squishlist
\item  \nodemoe consists of five node-experts and gating network to selectively pool node representations \hv to graph representation \hg:

\begin{align}
    \V{p} &= \V{M}(\V{h}_\V{V}) \nonumber \\
     \V{h}_\V{G} &= \sum_{v \in \V{V}} p_v E_v(v) 
    \label{eqn:moegraph}
\end{align}

\item \graphmoe contains two experts (graph expert and question expert) and a gating network to combine the graph representation \hg returned by \graphmoe and the query representation \hq:

\begin{align}
    \V{p} &= \V{M}([ \V{h}_\V{G}; \V{h}_\V{Q} ]) \nonumber \\
     \V{h}_\V{y} &= E_\V{G}(\V{h}_\V{G}) + E_\V{Q}(\V{h}_\V{Q})
    \label{eqn:moenodequery}
\end{align}

\squishend

$\V{h}_\V{y}$ is then passed to a 1-layer MLP to perform classification.
% \todo{We acknowledge that fixed nature of our graphs, Add runtime / parameter analysis.}





% \subsection{Graph convolutional network}


==> mercurie/sections-without-graphgen/comments_to_3.2.tex <==
We found that 70\% of the randomly sampled 100 graphs produced by \gnoisy had \textit{repeated} nodes \st{with overlapping information}. The repeated nodes introduce noise because they violate the semantic structure of a graph. From our experiments, we observed that modifying the training (from $x = P \Vert H \Vert S$ to $x=P \Vert H \Vert S \Vert T$) reduces repetitions \corr{significantly}{13\%}, we call this system \badtobetter. Since we do not have access to $T$ during test time, we \corr{train}{train a seq2seq model to generate} \betterg that takes where input=\badg and output=\betterg. 

During inference, for each defeasible input query we first use \gnoisy and then correct it via \badtobetter to get the final inference graph. We found that this process helped reduce repetitions by 13\% overall.



==> mercurie/sections-without-graphgen/conclusion.tex <==
\section{Conclusion} 
We present \ours, a system that achieves a new state-of-the-art on three different defeasible reasoning datasets. We find that primary reason for these gains is that \ours models the question scenario with an inference graph, and judiciously encodes the graph to answer the question. This result is significant, because it shows that performance can be improved by guiding a system to ``think about'' a question and explicitly model the scenario, rather than answering reflexively.


% \section*{Acknowledgments}
% This material is partly based on research sponsored in part by the Air Force Research Laboratory under agreement number FA8750-19-2-0200. 
% The U.S. Government is authorized to reproduce and distribute reprints for Governmental purposes notwithstanding any copyright notation thereon. 
% The views and conclusions contained herein are those of the authors and should not be interpreted as necessarily representing the official policies or endorsements, either expressed or implied, of the Air Force Research Laboratory or the U.S. Government.
% We would like to thank Google for providing the TPU machines for conducting experiments.

==> mercurie/sections-without-graphgen/introduction.tex <==
\section{Introduction}

Defeasible inference is a mode of reasoning where conclusions may be modified given additional information \cite{sep-reasoning-defeasible}.
Here we consider the specific formulation and challenge in \cite{rudinger-etal-2020-thinking}:
Given that some premise \pre plausibly implies a hypothesis \hypo, does
new information that the situation is \upd weaken or strengthen the conclusion \hypo?
For example, given ``The drinking glass fell'' weakly implies ``The glass broke'',
being told ``The glass fell on a pillow'' here {\it weakens} the implication.
% Great motivation for a possible work on generation \citet{rudinger-etal-2020-thinking} also show that if the currently best performing pre-trained language model on defeasible inference is asked to generate \upd given \pre and \hypo, then it suffers from two problems: (i) not staying on topic as they often ignore \pre. For instance, when the premise mentions picking up someone at the airport, but the update talks about driving them there. (ii) not drawing meaningful connections between \pre, \hypo, and \upd. For instance, in about 25\% of the predictions, \upd and \hypo or \upd and \pre were found to be repeated.


\begin{figure}
\centerline{
\fbox{
    \parbox{0.44\textwidth}{
    \centering
	\small{Prior work:  $x \rightarrow y$ \\
	\ours:  $h(x, g(x)) \rightarrow y$ \\}
	\vspace{2mm}
	\flushleft
    \squishlist
        \item[$x$:] \small{Given that ``The drinking glass fell''. Will it strengthen or weaken the hypothesis ``The glass broke'' suppose ``The glass fell on a pillow''.}
        \item[$y$:] weakens
        \vspace{2mm}
        \item[$g(x)$:] \small{Generated inference graph for ques. scenario $x$}
        {\includegraphics[width=0.40\textwidth]{mercurie/imgs/example-glass.png}}
        % \item[$f(.)$:] \small{Inference graph encoder with gating.}
    \squishend
    }
}}
\caption{\ours improves defeasible reasoning by modeling the question scenario \x with an inference graph $g(x)$ (available from \mclean dataset). The graph is encoded judiciously using our graph encoder $h(.)$, resulting in end task performance improvement.}
\label{fig:opening-overview}
\end{figure}

% inference graph here:
% https://aristo-demo-2019.apps.allenai.org/wiqa-ig?ig=%7B%0A%20%20%20%20"situations"%3A%20%7B%0A%20%20%20%20%20%20%20%20"Z"%3A%20%5B%20"C-%20%3A%20A%20person%20is%20sick"%20%5D%2C%0A%20%20%20%20%20%20%20%20"V"%3A%20%5B%20"C%2B%20%3A%20A%20person%20is%20healthy"%20%5D%2C%0A%20%20%20%20%20%20%20%20"X"%3A%20%5B%20"S%20%3A%20Person%20owns%20a%20shop"%5D%2C%0A%20%20%20%20%20%20%20%20"W"%3A%20%5B%20"M-%20%3A%20Person%20does%20not%20have%20to%20pay%20for%20medicine"%20%5D%2C%0A%20%20%20%20%20%20%20%20"U"%3A%20%5B%20"S-%20%3A%20Person%20is%20self-employed"%20%5D%2C%0A%20%20%20%20%20%20%20%20"Y"%3A%20%5B%20"M%2B%20%3A%20Person%20has%20full%20medical%20coverage"%20%5D%2C%0A%20%20%20%20%20%20%20%20"A"%3A%20%5B%20"H-%20%3A%20Person%20buys%20medicine"%20%5D%2C%0A%20%20%20%20%20%20%20%20"D"%3A%20%5B%20"H%2B%20%3A%20Person%20does%20not%20buy%20medicine"%20%5D%0A%20%20%20%20%7D%2C%0A%20%20%20%20"emphasizedEdges"%3A%20%5B%20"ZX"%2C%20"VX"%2C%20"XW"%2C%20"XY"%2C%20"UY"%2C%20"WD"%2C"YA"%20%5D%0A%7D



%  \begin{figure}[!h]
%                         {\includegraphics[scale=0.23]{mercurie/imgs/example-insurance.png}}
%                         % \caption{A sample inference graph for the running example.}
%                         \label{fig:fig1-subfig}
%                     \end{figure}

A desirable approach is to jointly consider \pre, \hypo, \upd to avoid deviating from the topic and to avoid repetition errors. We found that we can borrow ideas from the cognitive science literature that supports defeasible reasoning for humans with an \emph{inference graph} \citep{Pollock2009ARS}.  Inference graphs draw connections between the \pre, \hypo and \upd through mediating events. This can be seen as a \emph{mental model} of the question scenario before answering the question. This paper asks the natural question whether modeling the question scenario with inference graphs could help machines in defeasible reasoning? %\todo{keep the story like the abstract, also mention human helps paper}


\textbf{Proposed system}: Our approach is, given a question, to have a model first create an inference graph, and then use that graph as an additional input when answering the defeasible reasoning query. Our proposed system, \ours, comprises of a graph generation module, and a graph encoding module to use the generated graph for the query.


% \begin{figure}[!ht]
% \centering
% {\includegraphics[width=\columnwidth]{imgs/diagrams.pdf}}
% \caption{An overview of \ours}
% \label{fig:deftrain}
% \end{figure}


To generate inference graphs, we use past work that uses a sequence to sequence approach \cite{madaan2021improving}. Their model uses data augmentation to create like-gold graphs. However, the resulting graphs can often be erroneous, and so they included an error correction module to generate higher quality inference graphs. This was important because we found that better graphs are more helpful in the downstream QA task.

The generated inference graph is used for the QA task on three existing defeasible inference datasets from diverse domains, viz., \snli (natural language inference) \cite{bowman2015large}, \social (reasoning about social norms) \cite{forbes2020social}, and \atomic (commonsense reasoning) \cite{sap2019atsosomeomic}. We show that by simply augmenting the question with our generated  graphs, there are some gains on all datasets. Importantly, we show that with a more judicious  encoding of the graph augmented question that accounts for interactions between the graph nodes, the QA task accuracy improves substantially across all datasets. To achieve this, we use the mixture of experts approach \cite{mixture-of-experts-paper} to include mixture of experts layers during encoding, enabling the ability to selectively attend to certain nodes while capturing their interactions. 

In summary, our contribution is in borrowing the inference graph idea from cognitive science literature to show benefits in defeasible inference QA task. Using an error correction module in the graph generation process, and a judicious encoding of the graph augmented question, \ours achieves a new state-of-the-art over three defeasible datasets, as well as now producing justifications for its answers. 
This result is significant also because our work illustrates that performance can be improved by guiding a system to think about a question. This encourages future studies on other tasks, where the question scenario can be modeled first, rather than answering reflexively. 




==> mercurie/sections-without-graphgen/related_work.tex <==
\section{Related work}


% \paragraph{\pete{Self talk}} xxxxx TODO xxxxx

\paragraph{Mental Models} Cognitive science has long promoted mental models - coherent, constructed representations of the world - as
central to understanding, communication, and problem-solving \cite{JohnsonLaird1983MentalM,mental-models,Hilton1996MentalMA}.
Our work draws on these ideas, using inference graphs to represent the machine's ``mental model'' of the problem at hand.
Building the inference graph can be viewed as first asking clarification questions about the context before answering. This is similar to self-talk \cite{selftalk} but directed towards eliciting chains of influence, the inference graph template acting as a schema for a mental model.

\paragraph{Generating graphs for commonsense reasoning}
% \niket{For augmented QA, throwing in additional input may or may not help. But we need to know what to add and how. What to add is an inference graph that captures mediator and contextualizer events, in a joint setting, and relevant to the premise.}

The use of generated knowledge to aid question answering has recently gained much attention~\cite{bosselut2019dynamic, yang2020g,madaan2020eigen,rajagopal2021curie}.
\textsc{comet}~\cite{Bosselut2019COMETCT} uses \textsc{gpt}~\citep{radford2018improving} fine-tuned over commonsense knowledge graphs like \textsc{atomic}~\cite{sap2019atomic} and conceptnet~\citep{speer2017conceptnet} for KB completion.
Similarly, \citet{rajagopal2021curie} aim to generate event influences grounded in a situation using pre-trained language models.
Similar to these works, we adopt large-scale language models for such a conditional generation of text for commonsense reasoning. However, our graph generation method generates complete graphs, as opposed to a short event or phrase generated by these methods.


Information retrieval is another way of collecting necessary knowledge. Influences captured in inference graphs can also be disjointly generated via this approach, but it is non-trivial to preserve the joint semantics \pre, \hypo, \upd. \cite{brahman2020learning} generate rationales for defeasible inference, but it is done post-hoc i.e., given the answer they generate a rationale based on its training over e-SNLI corpus which is related to the $\delta$-NLI dataset. They found that their system mostly generates very trivial rationales. We address the more realistic setup of jointly predicting an inference graph and not in a post-hoc manner, which that paper suggested as an important future direction.

%e.g.,
% premise -> situation -> mediating -> hypothesis.
% we can ask IR/ event KG:
% what does premise lead to?
% what does situation lead to?
% what can lead to hypothesis?
% this would require some joint reasoning over the three answers.



% \am{Add a line comparing with \cite{defeasible-human-helps-paper}}
% Peter: The paper shows that pulling in influence graphs helps with QA, compared with simply doing QA. I guess another baseline would be: what alternative might you pull in that might help QA? e.g., some COMeT-generated facts, or some IR facts?   That's beyond the scope of what you can do for the EMNLP submission, but it's an interesting question about: Why influence graphs, specifically?

% Niket Tandon  5:03 PM
% Motivation for inference graphs is directly coming from cogsci literature  (second para in introduction).
% 5:03
% Its a reasonable way to connect PHU. But not the only way

% peterc  5:04 PM
% I suppose you could compare with injecting some weaker from of influence graphs, e.g., just the node sentences, but not the edges - although most of the nodes wouldn't reall ymake sense.
% 5:04
% I agree, the CogSci literature is a good basis for trying IGs
% 5:06
% In general, there are a bunch of ways one can inject CSK into a model; generally they seem to produce tiny-ish gains in the literature, but it's not a panacea - the open question is to know what background knowledge is best to inject, and how to inject it. IGs are a good conjecture to explore as an answer to this question.

% Niket Tandon  5:10 PM
% Yes. Also, mediating events can also be generated via IR/eventKG but it is non-trivial because the semantics between premise situation and hypothesis needs to be preserved. e.g.,
% premise -> situation -> mediating -> hypothesis.
% we can ask IR/ event KG:
% what does premise lead to?
% what does situation lead to?
% what can lead to hypothesis?
% this would require some joint reasoning over the three answers.

Our work is closest in spirit to \citet{bosselut2019dynamic} generate a tree that connects question to answer choices via an intermediate layer of generated nodes. As opposed to \citet{bosselut2019dynamic}, we do not perform on the fly generation of graph nodes, and instead directly consume a pre-generated graph.


% Learning generative models of graphs forms another existing line of research.
% Notable examples include \citet{you2018graphrnn}, who formulate graphs as a sequence for learning generative models of synthetic and real-world graphs.
% Other popular graph generation techniques employ a VAE~\cite{simonovsky2018graphvae} and graph-structure dependent decoding processes~\cite{li2018learning}.
% However, unlike these works which focus on learning generative distributions of graphs, our focus is conditional generation of commonsense graphs.

% We note that our graph generation process does not make any graph-specific assumptions and follows a sequence-to-sequence paradigm, following the recent success of these methods on complex tasks~\cite{raffel2020exploring,lewis2020bart}




\paragraph{Graph Neural Networks for commonsense QA}
Several existing methods use graphs as an additional input for commonsense reasoning~\cite{lin2019kagnet,lv2020graph,feng2020scalable}.
These methods first retrieve a graph relevant to a question using information retrieval techniques, and then encode the graph using graph representation techniques like~\gcn~\cite{kipf2016semi}.
Different from these works, we use a generated graph grounded in the query for answering commonsense question.
While we experiment with state-of-the-art \gcn models, our model improves over the \gcn based representations by using a mixture-of-experts (\moe)~\cite{jacobs1991adaptive} to pool multi-faceted input.
Prior work has looked at using \moe for graph classification tasks~\cite{zhouexplore}.
\citet{chen2019multi} use \moe to mix features from various languages for downstream POS and NER tagging tasks.
To the best of our knowledge, we are the first to use \moe to pool graph representations for a downstream \qa task.



==> mercurie/sections-without-graphgen/results.tex <==
\section{Experiments}
In this section we empirically study whether we can improve defeasible inference task by first modeling the question scenario using inference graphs. We also study the reasons for any improvements, and perform error analysis.

\subsection{Experimental setup}


\begin{table}[!ht]
\centering
%  \resizebox{\columnwidth}{!}{
\begin{tabular}{llrr}
\toprule
Dataset & Split & \# Samples & Total\\ \midrule
%  \multirow{3}{*}{\wiqa} & train & 1522 & \multirow{3}{*}{2107} \\
%       & test   & 189  \\
% & dev  & 152 \\ \midrule
 \multirow{3}{*}{\atomic} & train & 35,001 & \multirow{3}{*}{42,977} \\
      & test   & 4137  \\
& dev  & 3839 \\ \midrule
 \multirow{3}{*}{\social} & train & 88,675 & \multirow{3}{*}{92,295} \\
      & test   & 1836  \\
& dev  & 1784 \\ \midrule
 \multirow{3}{*}{\snli} & train & 77,015 & \multirow{3}{*}{95,795} \\
      & test   & 9438  \\
& dev  & 9342 \\
\bottomrule
\end{tabular}
% }
\caption{Number of samples in each dataset by split. 
% \atomic, \snli, \social are available at~\url{https://github.com/rudinger/defeasible-nli}, \wiqa is available at~\url{https://allenai.org/data/wiqa} . \niket{instead of \wiqa, describe dataset in human helps paper}
}
\label{table:data-split}
\end{table}

\paragraph{Datasets}
Our end task performance is measured on three existing datasets for defeasible inference\footnote{ \url{github.com/rudinger/defeasible-nli}}: \atomic, \snli, \social. Table \ref{table:data-split} presents the statistics. These datasets exhibit substantial diversity because of their domains : \snli (natural language inference), \social (reasoning about social norms), and \atomic (commonsense reasoning). It would require a general model to perform well across these diverse datasets.








\paragraph{Baselines and setup}
The previous state-of-the-art (SOTA) is the \roberta~\cite{liu2019roberta} model presented in \citet{rudinger-etal-2020-thinking}, and we report the published numbers for this baseline. We adhere to the same hyperparameters used in that paper for \lm used in \ours. For more hyperparameter details for \ours, we refer to the Appendix.  %by \citet{rudinger-etal-2020-thinking}.
% Recall that we have three versions of graphs corresponding to each defeasible query: \GEN, \CORR, \CORWF. 
% \niket{TODO: implementation details}

% Now this doesn't make sense here.
% \paragraph{Methods}
% We experiment with three different ways of learning graph representations: vanilla string-based (\str~\secref{sec:string_pooling}), \gcn based (\secref{sec:gcn_pooling}), and finally \moe based (\secref{sec:moe_pooling}).




\subsection{Results}
\label{sec:rq2}
Table \ref{tab:overall-main-result} compares QA accuracy on these datasets without and with modeling the question scenario with our generated graphs. The results suggest that we get consistent gains across all datasets. \snli sees the highest gains. \ours achieves a new state-of-the-art on all three different datasets, as well as now producing justifications for its answers.
% The relatively smaller gains on \atomic can be attributed to the comparatively higher noise in \atomic (\cite{rudinger-etal-2020-thinking} show that humans disagreed on the question correctness nearly twice more than for other datasets).


\newcommand{\tabw}{1.61cm}
\begin{table}[!t]
\centering
\begin{tabular}{p{1.59cm}p{\tabw}p{\tabw}p{\tabw}p{\tabw}}
\toprule
 & \atomic & \snli & \social \\
\midrule
\small{Prev-SOTA}   & 78.3\ \textpm\ 1.3   & 81.6\ \textpm\ 1.8 & 86.2\ \textpm\ 0.7  \\
\ours &   \textbf{80.2}\ \textpm\ 1.2  & \textbf{85.6}\ \textpm\ 1.7 & \textbf{88.6}\ \textpm\ 0.7  \\
\bottomrule
\end{tabular}
\caption{\ours is better on multiple domains on defeasible inference. Demonstrates  self-thinking on ques through generating an inference gr. helps. All the results are statistically significant with $p < 0.005$ using the sign-test and McNemar's test.\footnote{We add the p-values in the Appendix Table~\ref{tab:statanalysis}}}
\label{tab:overall-main-result}
\end{table}

% We primarily attribute these gains to the graph encoding scheme in the form of a \moe, which allows learning good quality graph representations. 
We study the reasons behind these gains by analyzing the contributions of the graph quality and the graph encoder. 

% The following detail will add confusion so commenting it. This is already incorporated in some form in the why gains subsection.
% Our experiments span two types of graphs  (\GEN, \CORWF), three datasets (\snli, \social, \atomic), and three graph encoding schemes (\str, \gcn, \moe). In the interest of space and clarity, we defer the numbers on all 18 combinations of $\{\text{graph types}\} \times \{\text{datasets}\} \times \{\text{graph encoding schemes}\}$  to the appendix.
% $\{\C{G}_{\text{good}} \times \C{G}_{\text{bad}} \} \times \{\text{\textsc{atomic}}, \text{\textsc{snli}}, \text{\textsc{social}}\} \times  \{\text{\textsc{str}}, \text{\textsc{gcn}}, \text{\textsc{rgcn}}, \text{\textsc{moe}}\}$
% Here, we verify our claim of the source of gains by first comparing our best method (\moe) over the two graph types (\GEN and \CORWF) in Section~\secref{sec:graph_quality_gains}.
% Next, in Section~\secref{sec:graph_encoding_gains}, we compare various graph encoding schemes over good graphs, and show that \moe defeats the other schemes by a large margin.


% \am{
% \squishlist
%     \item Add confidence intervals.
%     \item Add statistical significance test.
% \squishend
% }



\label{sec:results}






\subsection{Understanding \ours gains}
In this section, we study the contribution of the main components of the \ours pipeline. %, namely graph corrector and graph encoder. 

% \subsubsection{graph quality: good graphs, better downstream performance?}
% \label{sec:graph_quality_gains}


% \paragraph{Do more informative graphs lead to a better downstream performance?}
% \paragraph{Effect of graph quality on downstream task?}
\subsubsection{Impact of graph correctness:}

As previously mentioned, the authors of \mercurie provide two datasets: \mclean and \mnoisy. To study whether graph correctness is important, we switch \mclean with \mnoisy as input to \ours's graph encoder. Table~\ref{tab:better_graphs_better_perf} shows that this consistently hurts across all the datasets. This indicates that noisier graphs lead to worse task performance, and better graphs improve performance. 

\begin{table}[!h]
\centering
\begin{tabular}{lrrr}
\toprule
 & \atomic & \snli & \social \\
\midrule
\GEN  & 78.5\  \textpm\ 1.3 & 83.8\  \textpm\ 1.8& 88.2\ \textpm\ 0.7  \\
\CORWF &   \textbf{80.2}*\ \textpm\ 1.2  & \textbf{85.6}*\ \textpm\ 1.7 & \textbf{88.6}\ \textpm\ 0.7    \\
% \ours - Graph correction &  xxx  & xxx & xxx  \\
% \ours - Graph encoding   &  xxx  & xxx & xxx  \\
\bottomrule
\end{tabular}
\caption{Better graphs lead to better task performance. * indicates statistical significance with $p < 0.02$.}
\label{tab:better_graphs_better_perf}
\end{table}


% \paragraph{Are graphs corrected by \CORR less noisy?}
% Recall that in this work, noise is defined as repetitions in the graph. We evaluate the repetitions in the graphs produced by \GEN and \CORR using two metrics: (i) repetitions per graph: average number of repeated nodes in a graph. (ii) \% with repetitions: percentage of graphs with at least one repeated node.


% \begin{table}[!h]
% \centering
% \begin{tabular}{ll|ll}
% \hline
%         & Repetitions & \GEN & \CORWF \\ \hline
% \atomic & per graph            & 2.05 & \textbf{1.26}   \\ \cline{2-4} 
%         & \% graphs            & 72   & \textbf{48 }    \\ \hline
% \snli   & per graph            & 2.09 & \textbf{1.18}   \\ \cline{2-4} 
%         & \% graphs            & 73   & \textbf{46}     \\ \hline
% \social & per graph            & 2.2  & \textbf{1.32}   \\ \cline{2-4} 
%         & \% graphs            & 75   & \textbf{49}     \\ \hline
% \end{tabular}
% \caption{\CORR reduces the inconsistencies in the graphs. The number of repetitions on average per graph and percentage of graphs with some repetition, both improve. }
% \label{tab:graph-gcorr-noise-reduces}
% \end{table}


% As Table~\ref{tab:graph-gcorr-noise-reduces} shows, \CORR reduces repetitions by approximately 40\% (2.11 to 1.25) across all datasets, and also reduces the fraction of graphs with at least one repetition by $~$25.7\% across .





% \begin{table}[!h]
% \centering
% \begin{tabular}{lrr}
% \toprule
%         & \GEN  & \CORWF \\ \midrule
% \atomic & 78.54 & 79.14  \\
% \snli   & 83.83 & 85.59  \\
% \social & 88.23 & 88.62  \\
% \bottomrule
% \end{tabular}
% \caption{Better graphs lead to better downstream performance.}
% \label{tab:better_graphs_better_perf}
% \end{table}



% \subsubsection{Effect of graph pooling on downstream task}
\subsubsection{Impact of graph encoder:}
\label{sec:graph_encoding_gains}
% \paragraph{Is \moe the best way to pool node representations}

% \paragraph{Baselines for graph encoding}
% The second method builds upon state-of-the-art method by~\cite{lv2020graph} for learning graph representation using graph convolutional networks and self-attention. We describe each of these in turn next.
We experiment with two alternative approaches to graph encoding to compare our \moe approach:

\begin{enumerate}

\item \textbf{Graph convolutional networks}: We follow the approach of \citet{lv2020graph} who use  \gcn~\cite{kipf2016semi} to learn rich node representations from graphs. Broadly, node representations are initialized by \lm and then refined using a \gcn. Finally, multi-headed attention~\cite{vaswani2017attention} between question representation \hq and the node representations is used to yield \hg. We add a detailed description of this method in (Appendix~\secref{sec:gcn_pooling}).

\item \textbf{String based representation}: Another popular approach \cite{proscript,madaan2020neural} is to concatenate the string representation of the nodes , and then using \lm to obtain the graph representation \hg$=\C{L}(v_1 \| v_2 \| .. )$ where $\|$ indicates string concatenation. 

\end{enumerate}

Table~\ref{tab:better_encoding_better_perf_1}  shows that \moe graph encoder is instrumental in enhancing end task performance, with only 5\% additional parameters introduced compared to the \str baseline (see Table \ref{tab:tradeoffs}). Next, we study the reasons for these gains. %\todo{move it up}


We suspect that the lacking performance of \gcn is because of the inability of \gcn to ignore the noise present in the graphs.
The graphs augmented with each query are not human-curated, and are instead generated by a language model in a zero-shot inference setting. Thus, the \gcn style message passing instead might amplified the noise in graph representations. 
On the other hand, \nodemoe first selects the nodes that are most useful to answer the query in order to form the graph representation \hg.
Further, \graphmoe can decide to completely discard the graph representations, as it does in a lot of the cases where the true answer for the defeasible query is weakener.

To further establish the possibility of message passing hampering the downstream task performance, we experiment with a \gcn-\moe hybrid, wherein we first refine the node representations using a 2-layer \gcn as used by \cite{lv2020graph}, and then pool the node representations using an \moe.
We found the results to be about the same as ones we obtained with \gcn~Table~\ref{tab:hier_moe_gcn}, indicating that bad node representations are indeed the root cause for the bad performance of \gcn. This is also supported by  \cite{Shi2019FeatureAttentionGCNUnderNoise} that found that noise propagation directly deteriorates network embedding and \gcn is not senstive to noise.
% \todo{support the claim that noise propagation amplifies noise with a citation. \url{https://arxiv.org/pdf/1912.11755.pdf}}
% When noise is imposed to the node (e.g. incorrect words), it will force existing methods, such as GCN or attention networks, to learn deteriorated weight values, corresponding to noisy features. Such noise propagation directly deteriorates network embedding results as we will show in Section 5


\begin{table}[!ht]
\centering
\begin{tabular}{lr} \toprule
Dataset & accuracy \\ \midrule
\atomic & 78.69 \\
\snli & 84.3 \\
\social &  87.76 \\ \bottomrule
\end{tabular}
\caption{Ablation: using an \moe on top of \gcn refined representations hurts performance.}
\label{tab:hier_moe_gcn}
\end{table}



Interestingly, graphs help the end-task even when encoded using a relatively simple \str based encoding scheme, further establishing their utility.















\begin{table}[!h]
\centering
\begin{tabular}{lrrr}
\toprule
 & \atomic & \snli & \social \\
\midrule
\str & 79.5\ \textpm\ 1.3  & 83.1\ \textpm\ 1.8 & 87.2\ \textpm\ 0.7  \\
\gcn & 78.9\ \textpm\ 1.3  & 82.4\ \textpm\ 1.8 & 88.1\ \textpm\ 0.7  \\
\moe  &  \textbf{80.2}\ \textpm\ 1.2  & \textbf{85.6}\ \textpm\ 1.7 & \textbf{88.6}\ \textpm\ 0.7    \\
\bottomrule
\end{tabular}
\caption{Contribution of \moe based graph encoding compared with alternative graph encoding methods. The gains of \moe over \gcn are statistically significant for all the datasets with $p < 0.02$, and the gains over \str are significant for \snli and \social with $p < 1e-05$.}
\label{tab:better_encoding_better_perf_1}
\end{table}



% \niket{what about graph corrector module?}
\begin{table}[!h]
\centering
\begin{tabular}{lll} \toprule
Method & \#Params & Runtime   \\ \midrule
\str & 124M & 0.17 \\
\gcn & 131M &  0.47  \\
\moe & 133M & 0.40  \\ \bottomrule
\end{tabular}
\caption{Number of parameters in the different encoding methods. Runtime reports the number of seconds to process one training example.}
\label{tab:tradeoffs}
\end{table}





% \begin{table}[!h]
% \centering
% \begin{tabular}{lrrr}
% \toprule
%  & \atomic & \snli & \social \\
% \midrule
% \str & 79.5  & 83.1 & 87.2  \\
% \gcn & 78.9  & 82.4 & 88.1  \\
% % \rgcn & 78.7  & 82.8 &  88.2   \\
% \moe  &   \textbf{80.2}  & \textbf{85.6} & \textbf{88.6}  \\
% % \ours - Graph correction &  xxx  & xxx & xxx  \\
% % \ours - Graph encoding   &  xxx  & xxx & xxx  \\
% \bottomrule
% \end{tabular}
% \caption{A comparison of various methods to encode the graph for the defeasible end task.}
% \label{tab:better_encoding_better_perf_2}
% \end{table}















\subsubsection{Detailed \moe analysis}
We now analyze the \moe used in \ours: (i) the \moe over the nodes i.e, \nodemoe, and (ii) the \moe over $\V{G}$ and input $x$ i.e., \graphmoe. 

%[width=0.90\textwidth,height=0.25\textheight]
\begin{figure}[!ht]
\centering
{\includegraphics[width=0.40\textwidth,height=0.22\textheight]{imgs/graph_ques_moe_gate_dist.pdf}}
\caption{\graphmoe gate values for the classes strengthens and weakens, averaged over the three datasets.}
\label{fig:graphquesmoedist}
\end{figure}

\paragraph{\graphmoe performs better for $y=$strengthens:} Figure~\ref{fig:graphquesmoedist} shows that the graph makes a comparatively contribution than the input, when the label is strengthen. In instances where the label is weakener, the gate of \graphmoe gives a higher weight to the question. This trend was present across all the datasets. We assume this happens because language models are tuned to generate events that happen rather than events that don't. In case of a weakener, the nodes must be of the type event1 leads to less of event2, whereas language models are naturally trained for event1 leads to event2. This requires further investigation in the future.  %\todo{when people write defeasible query, it's usually positive} 



% The following section seems to be missing, so commented it?
% Please see Section~\secref{sec:inferenceinfluencemapping} for a detailed description of these terms.
\paragraph{\nodemoe relies more on certain nodes:} We study the distribution over the types of nodes and their contribution to \nodemoe. Recall from Figure \ref{fig:moe} that C- and C+ nodes are contextualizers that provide more background context to the question, and S- node is typically an inverse situation (i.e., inverse \upd), while M- and M+ are the mediator nodes leading to the hypothesis. Figure \ref{fig:nodemoedist} shows that the situation node S- was the most important. This is followed by the contextualizer, and the mediator.
% (which was only used by \atomic). \niket{Why does atomic use mediators.} 
Notably, our analysis shows that mediators are less important for machines than they were for humans in the experiments conducted by~\cite{defeasible-human-helps-paper}. This is possibly because humans and machines may use different pieces of information. As our error analysis will later show in \S{\ref{sec:analysis}}, the mediators can be redundant given $x$. Humans might have used the redundancy to reinforce their beliefs, whereas machines leverage the unique signals present in S- and the contextualizers to solve the task. 

\begin{figure}[!ht]
\centering
{\includegraphics[width=0.48\textwidth]{mercurie/imgs/node_moe_gate_dist.pdf}}
\caption{\nodemoe gate values for the three datasets.}
\label{fig:nodemoedist}
\end{figure}



\paragraph{\nodemoe learns the node semantics:}  The network learned the semantic grouping of the nodes (contextualizers, situation, mediators) which became evident when plotting the correlation between the gate weights. There is a strong negative correlation between the situation nodes and the context nodes, indicating that only one of them is activated at a time.

% SORRY, this has to go. It is adding limited information. We can express in words.
\begin{figure}[!ht]
\centering
{\includegraphics[width=0.48\textwidth,height=0.20\textheight]{mercurie/imgs/gate_corr.pdf}}
\caption{Correlation between probability assigned to each semantic type of the node by \nodemoe}
\label{fig:gatecorr}
\end{figure}

\paragraph{\nodemoe, \graphmoe have a peaky distribution:} Ideally, a peaky distribution over the gate values (low entropy) is desired, as it implies that the network is judiciously selecting the right expert for a given input. We compute the average entropy of \nodemoe and \graphmoe and found the entropy values to be low~(Table~\ref{tab:entropy}), which indicates a peaky distribution.
These peaky distribution over nodes can be considered as an explanation through supporting nodes. This is analogous to scene graphs based explanations in visual QA \cite{Ghosh2019VQAExplanations}.  

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[!ht]
\centering
\begin{tabular}{lcc}
\toprule
Gate  & Uniform entropy & \moe Entropy     \\ \midrule
\nodemoe  & 2.32 & 0.52  \\
\graphmoe & 1.0 & 0.08  \\ \bottomrule
\end{tabular}
\caption{Entropy values for \nodemoe and \graphmoe calculated using $\log_2$. Low entropy values are desired, and indicate higher selectivity. %The maximum possible entropy is listed in the parenthesis. 
}
\label{tab:entropy}
\end{table}

% \todo{highlight explainability}. (highlighted.)
% and found that the  is worst for atomic. Correlation b/w end task and node + graph/ques selection, more fuzzy -> less qa acc [Remark in MOE effectiveness + appendix diagram] 


% Note: this combination of gcn and moe is not important. We don't exactly know why.
% Moving this comment to here.
% \am{We also tried combining gcn + moe, but it gave suboptimal results (show numbers)}
% \am{GCN will be hurt by 0 shot graphs, as there is a propagation/amplification of noise from one node to another.}












% \subsubsection{Detailed \moe analysis}
% We now explore the reasons for these gains by \moe by performing an analysis of the gates of two MOEs: i) \nodemoe, and ii) \graphmoe 

% \squishlist
% \item  As Figure~\ref{fig:graphquesmoedist} shows, for strengtheners, the graph plays a more important role than the question. The situation is reversed for weakeners, where the gate of \graphmoe gives a higher weight to the question. We posit that this stems from the inability of language models to generate convincing events in the graph for weakeners (or attenuators)~\todo{citation}. We found that this trend was present across the datasets.\todo{when people write defeasible query, it's usually positive}

% %[width=0.90\textwidth,height=0.25\textheight]
% \begin{figure}[!ht]
% \centering
% {\includegraphics[width=0.40\textwidth,height=0.22\textheight]{imgs/graph_ques_moe_gate_dist.pdf}}
% \caption{\graphmoe gate values for the classes strengthens and weakens, averaged over the three datasets.}
% \label{fig:graphquesmoedist}
% \end{figure}

% \todo{Why is \gcn not working?}
% \item Figure \ref{fig:nodemoedist} shows the distribution over the node classes over the three datasets. Please see Section~\secref{sec:inferenceinfluencemapping} for a detailed description of these terms.
% As expected, the situation node was the most important, followed by the contextualizer, followed by the mediator (which was only used by \atomic). Further, we observed that for the cases that were corrected by  is flipped to correct, the average mediator probabilities go up from 0.09 to 0.13 averaged over the datasets.
% Notably, our analysis shows that mediators are less important for machines than they were for humans in the experiments conducted by~\cite{defeasible-human-helps-paper}.
% This underscores the fact that humans and machines may use different pieces of information.
% As our error analysis shows, the mediators typically contained information that is redundant given \dquery. 
% Humans might have used the redundancy to reinforce their beliefs, whereas the machines leverage the unique signals present in the situation and the contextualizers to solve the task. 

% \begin{figure}[!ht]
% \centering
% {\includegraphics[width=0.48\textwidth,height=0.20\textheight]{mercurie/imgs/node_moe_gate_dist.pdf}}
% \caption{\nodemoe gate values for the three datasets. \niket{is this gate MOE?} - it is not super clear}
% \label{fig:nodemoedist}
% \end{figure}



% \item We also found that the network learned the semantic grouping of the nodes (contextualizers, situation, mediators) by plotting the correlation between the gate weights. As Figure~\ref{gatecorr} shows, there is a strong negative correlation between the situation nodes and the context nodes, indicating that only one of them is activated at a time.
% \begin{figure}[!ht]
% \centering
% {\includegraphics[width=0.48\textwidth,height=0.20\textheight]{mercurie/imgs/gate_corr.pdf}}
% \caption{Correlation between probability assigned to each semantic type of the node by \nodemoe}
% \label{fig:gatecorr}
% \end{figure}

% \item  Finally, we analyze the average entropy of the \nodemoe and \graphmoe.
% Ideally, a peaky distribution over the gate values (low entropy) is desired, as it implies that the network is judiciously selecting the right expert for a given input. \todo{Add exact entropy values} \todo{highlight explainability}.
% % and found that the  is worst for atomic. Correlation b/w end task and node + graph/ques selection, more fuzzy -> less qa acc [Remark in MOE effectiveness + appendix diagram] 
% \squishend

% % Moving this comment to here.
% \am{We also tried combining gcn + moe, but it gave suboptimal results (show numbers)}
% \am{GCN will be hurt by 0 shot graphs, as there is a propagation/amplification of noise from one node to another.}





















